Density Ratio Estimation via Infinitesimal Classification

Density ratio estimation (DRE) is a fundamental machine learning technique for comparing two probability distributions. However, existing methods struggle in high-dimensional settings, as it is difficult to accurately compare probability distributions based on finite samples. In this work we propose DRE-\infty, a divide-and-conquer approach to reduce DRE to a series of easier subproblems. Inspired by Monte Carlo methods, we smoothly interpolate between the two distributions via an infinite continuum of intermediate bridge distributions. We then estimate the instantaneous rate of change of the bridge distributions indexed by time (the "time score") -- a quantity defined analogously to data (Stein) scores -- with a novel time score matching objective. Crucially, the learned time scores can then be integrated to compute the desired density ratio. In addition, we show that traditional (Stein) scores can be used to obtain integration paths that connect regions of high density in both distributions, improving performance in practice. Empirically, we demonstrate that our approach performs well on downstream tasks such as mutual information estimation and energy-based modeling on complex, high-dimensional datasets.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%
\usepackage{amsmath,amsfonts,amsthm,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> my_macros.tex <==
% \newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\punbias}{p_{\rm{ref}}}
\newcommand{\pbias}{p_{\rm{bias}}}
\newcommand{\pdre}{p_{\rm{DRE}}}
\newcommand{\Dbias}{{\mathcal{D}_{\mathrm{bias}}}}
\newcommand{\Dunbias}{{\mathcal{D}_{\mathrm{ref}}}}
\newcommand{\Dp}{{\mathcal{D}_P}}
\newcommand{\Dq}{{\mathcal{D}_Q}}
\newcommand{\Sbias}{{\mathcal{S}_{\mathrm{bias}}}}
\newcommand{\Sunbias}{{\mathcal{S}_{\mathrm{ref}}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\bbR}{{\mathbb{R}}}
\newcommand{\bbE}{{\mathbb{E}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bw}{{\mathbf{w}}}

\def\iid{i.i.d\onedot}

==> rebuttal/cmd.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,amssymb,mathtools,amsthm}
\usepackage{color,xcolor}

\usepackage{hyperref}       % hyperlinks
\hypersetup{
  colorlinks,
  linkcolor={red!50!black},
  citecolor={blue!50!black},
  urlcolor={blue!80!black}
  }
  \definecolor{orange}{HTML}{ff7f0e}
  \definecolor{blue}{HTML}{1f77b4}
  
\usepackage{url}

\usepackage{algorithm}
\usepackage{adjustbox}
%\usepackage[noend]{algpseudocode}
% \usepackage{algpseudocode}
% \usepackage{algorithmicx}

\usepackage{microtype}
\usepackage{lipsum}
\usepackage{graphicx}
%\usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{sidecap}
\usepackage{caption}
\usepackage{booktabs} % for professional tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{comment}
\usepackage{enumitem}
\usepackage{wrapfig,tikz}
\usepackage{longtable,fancyhdr}
\usepackage{adjustbox, bigstrut, tabularx, multirow, makecell, diagbox}
\usepackage{graphicx,float}
\usepackage{stackrel}
\usepackage{color}
\usepackage{colortbl}
\usepackage{theoremref}
\usepackage{cases}
\usepackage{stmaryrd}
\usepackage{mathabx}
\usepackage{dsfont}

\usepackage[capitalise]{cleveref}


\makeatletter
\usepackage{xspace} 
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}

\definecolor{blue1}{RGB}{0,128,255}
\definecolor{blue3}{RGB}{0,0,128}
\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand*{\tran}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}

\def\eg{\emph{e.g}\onedot}
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot}
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot}
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot}
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\aka{a.k.a\onedot}
\def\iid{i.i.d\onedot}
\def\etal{\emph{et al}\onedot}

\definecolor{darkgreen}{rgb}{0,0.6,0}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}
\newcommand{\dotsim}{\mathrel{\dot{\sim}}}


% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vpi{{\bm{\pi}}}
\def\vomega{{\bm{\omega}}}
\def\vlambda{{\bm{\lambda}}}
\def\vphi{{\bm{\phi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\dt}{\frac{\partial}{\partial t}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}

\newcommand{\ud}{\mathrm{d}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}


\let\ab\allowbreak

\newcommand{\Dp}{{\mathcal{D}_P}}
\newcommand{\Dq}{{\mathcal{D}_Q}}
\newcommand{\bbR}{{\mathbb{R}}}
\newcommand{\bbE}{{\mathbb{E}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bff}{{\mathbf{f}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\dd}{{\textrm{d}}}

\newcommand{\dreinf}{{\textrm{DRE-}\infty}}

==> sections/acks.tex <==
\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> sections/method_v2.tex <==
\section{\kristy{testing} Time Score Matching via Infinitesimal Classification}
\label{time_training}
Recall that our motivation was to generalize TRE by taking the number of intermediate bridge distributions $T$ to the infinite limit.
With an infinite number of bridges, each intermediate classifier is tasked with distinguishing samples from two bridge distributions $p_{t+\Delta t}(\rvx)$ and $p_{t}(\rvx)$.
In fact, the following proposition states that the optimal form of this infinitesimal classifier 
is given by the time score $\dt \log p_t(\rvx)$.
\begin{proposition}
\label{prop:score_clf} When $T \rightarrow \infty$, the Bayes-optimal
% \se{is this the bayes-optimal?}\ys{Yes}
classifier between two adjacent bridge distributions $p_{t/T}(\rvx)$ and $p_{(t+1)/T}(\rvx)$ for any $t \in [0,1]$ is: 
\begin{equation}
    % \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} O\left(\dt \log p_t(\rvx)\right).
    \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} \left(\dt \log p_t(\rvx)\right) \Delta t + o(\Delta t).
\end{equation}
\end{proposition}
% \se{is this for any $t$?}\ys{Yes}
% \se{double check the statemetn of this proposition. deltaT goes to zero in the limit}
where $\Delta t = \frac{1}{T}$, 
and $\vh_{\vtheta^*}(\rvx, t) \in [0,1]$ is a conditional 
probabilistic classifier. 
% \kristy{is this accurate?}
% \ys{Need to mention somewhere that the big O is with respect to $\Delta t = 1/T$.}
% \se{big O notation doesn't make sense}

While the above result is instructive, it does not provide us with a practical algorithm for time score estimation---
we cannot train an infinite number of such binary classifiers.
% \kristy{This is important because the identity in \cref{sum_to_integral} has conveniently converted the need to solve $T$ binary classification problems into one that requires the ability to estimate the time scores.}
% \se{give some intuition here. $\frac{\partial}{\partial t} \log p_t(\rvx) \approx \log p_{t+\delta_t}(\rvx)  - \log p_{t}(\rvx) = \log \frac{p_{t+\delta_t}(\rvx)} {p_{t}(\rvx)} $}
% This expression says that the form of the optimal infinitesimal classifier becomes an expression of how much each intermediate density is changing over time ($\dt \log p_t(\rvx)$). 
% In direct analogy to traditional data (Stein) scores $\nabla_\rvx \log p(\rvx)$, we name this quantity $\dt \log p_t(\rvx)$ the \emph{time score} function of $p_t(\rvx)$.
% The above proposition immediately suggests that we may be able to train a time score model \kristy{todo}$\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$. 
% To do so, 
To tackle this challenge,
we consider the limit of the binary cross-entropy loss function for the optimal infinitesimal classifier (\cref{prop:score_clf}) when $T\to \infty$.
% \ys{Missing a constant in the expression?} \kristy{which constant where?}
\begin{proposition}
\label{prop:opt_clf}
Let $\Delta t = 1/T$ and parameterize the binary classifier as $\vh_\vtheta(\rvx, t) = \frac{1}{2} + \frac{1}{4} \vs_\vtheta^{\textrm{time}}(\rvx, t)\Delta t$, where $\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$ denotes a time score model. Then from the binary cross-entropy objective:
\begin{equation}
% \label{eq:loss}
\resizebox{\linewidth}{!}{$
\begin{split}
    &\arg \max_{\theta} \mathbb{E}_{p_{t}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t))] + \mathbb{E}_{p_{t+\Delta t}(\rvx)}[\log \vh_\vtheta(\rvx, t)]\\
    =& \arg \max_{\theta} -\frac{1}{4} (\Delta t)^2 \mbb{E}_{p_t(\rvx)}\left[\left(\vs_\vtheta^{\textrm{time}}(\rvx, t) - \dt \log p_t(\rvx) \right)^2\right] + o((\Delta t)^2)
\end{split}
$}
\end{equation}
\end{proposition}
We defer the proof to Appendix~\ref{pf-opt-clf}. 
% Notably, the form of the objective function in \cref{prop:opt_clf} exactly mirrors that of \cref{time_obj}, drawing the equivalence between solving an infinite number of ``infinitesimal'' classification problems and time score matching.

% We propose to train a time score model $s_\vtheta^{\textrm{time}}(\rvx, t)$ to estimate the true time scores $\dt \log p_t(\rvx)$ via the following objective:
Therefore, we see that the training of this infinitesimal classifier naturally lends itself to the following time score matching objective. We use this expression to train a time score model:
% In fact, we can further simplify \cref{prop:opt_clf}
% \ys{As the number of bridge distributions increase to infinity, $T\to \infty$ and therefore $\Delta t \to 0$, in which case certain terms can be dropped in the loss function...} We can use the following expression
% We use this expression 
% to obtain the 
% following objective for training a time score model $s_\vtheta^{\textrm{time}}(\rvx, t)$:
\begin{equation}
\label{time_obj}
\resizebox{\linewidth}{!}{$
\begin{split}
        \mathcal{J_{\text{time}}(\theta)} &= \E_{p(t)}\E_{p_t(\rvx)}\bigg[\lambda(t) \left( \dt \log p_t(\rvx) - s_\vtheta^{\textrm{time}}(\rvx, t) \right)^2 \bigg]
\end{split}
$}
\end{equation}
% \se{need to provide some guidance to the reader, the key issue is that the true score is unknown, so the objective cannot be evaluated let alone optimized}
% \se{it's also not clear why we needed to talk about $\vh_{\vtheta^*}(\rvx, t)$, since then it's not used anymore. why is the score model also parameterized by theta? }
where $\lambda(t): [0,1] \rightarrow \bbR_+$ is a positive weighting function and $p(t)$ is the uniform distribution over timescales.
While this objective is clearly minimized when $s_\vtheta^{\textrm{time}}(\rvx, t) = \dt \log p_t(\rvx)$, it might 
% \ys{Need to remind reader what $p(t)$ is}
Then using integration by parts as in \citep{hyvarinen2005estimation}, 
% we can show that 
this objective
% for learning $\dt \log p_t(\rvx)$ 
can be simplified to the following expression in \cref{prop:time_objective}.
As used in traditional score matching techniques \citep{kingma2010regularized,song2020sliced,song2019generative}, integration by parts allows us to obtain a practical objective function for training  $s_\vtheta^{\textrm{time}}(\rvx, t)$ that does not depend on the true time scores $\dt \log p_t(\rvx)$. 

\begin{proposition}[Informal]
\label{prop:time_objective}
Under certain regularity conditions, the optimal solution $\theta^{*}$ of \cref{time_obj} is the same as the optimal solution of
\begin{equation}
\resizebox{\linewidth}{!}{$
\begin{split}
        &\mathcal{L_{\text{time}}(\theta)} = 2 \E_{q(\rvx)}[\lambda(0) s_\vtheta^{\textrm{time}}(\rvx, 0)] - 2\E_{p(\rvx)}[\lambda(1) s_\vtheta^{\textrm{time}}(\rvx, 1)] \\
    &+\E_{p(t)}\E_{p_t(\rvx)}\bigg[2 \lambda(t) \dt s_\vtheta^{\textrm{time}}(\rvx, t) + 2\lambda'(t) s_\vtheta^{\textrm{time}}(\rvx, t) + \lambda(t) s_\vtheta^{\textrm{time}}(\rvx, t)\bigg]
\end{split}
$}
\end{equation}
\end{proposition}
where the first two terms of \cref{prop:time_objective} denote the boundary conditions for $t=\{0,1\}$, and the expectations can be approximated via Monte Carlo. 
Our ability to estimate the objective via Monte Carlo samples makes training $\dreinf$
% the training procedure of $\dreinf$ 
much more efficient than TRE, which requires the explicit construction of $T$ additional batches per gradient step for all intermediate classifiers.
% intermediate classifier. \kristy{reword}
% \kristy{This gives us a nice objective that we can work with in practice.}
We defer the exact assumptions and proof to Appendix~\ref{pf-time-prop}, and provide pseudocode in Appendix~\ref{app-pseudo}.

The optimal time score model, denoted by $s_{\vtheta^\ast}^{\textrm{time}}(\rvx, t)$, satisfies $s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$. Therefore after training, the log-density-ratio can be estimated by:
\begin{equation}
    \label{eqn:dr1}
    \log r(\rvx) \approx \int_{1}^0 s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \ud t. 
\end{equation}
% \begin{align*}
%     \label{eqn:dr1}
%     \log r(\rvx) \approx \int_{1}^0 s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \ud t.
% \end{align*}
using any numerical integrator as in \cref{sum_to_integral}.

\subsection{Joint Training Objective}
We can also incorporate
helpful auxiliary information from the data scores
into the training objective in \cref{time_obj}.
Specifically, we can define a vector-valued score model $\vs_\vtheta^{\textrm{joint}}(\rvx, t)$ and train it with a hybrid objective that seeks to \emph{jointly learn} $\nabla_{[\rvx; t]} \log p(\rvx, t)$:
\begin{equation}
\label{eqn:joint_obj}
\resizebox{\linewidth}{!}{$
        \mathcal{J_{\text{joint}}(\theta)} =
        \E_{p(t)}\E_{p_{t}(\rvx)}\left[ \frac{1}{2}\lambda(t)\norm{\nabla_{[\rvx; t]}\log p(\rvx, t) - \vs_\vtheta^{\textrm{joint}}(\rvx, t)}_2^2 \right].
$}
\end{equation}
The data score component in \cref{eqn:joint_obj} can be obtained by DSM \citep{vincent2011connection} or SSM \citep{song2020sliced}.
For the SSM variant, \citep{hyvarinen2005estimation,song2020sliced} shows that optimizing \cref{eqn:joint_obj} is equivalent to the optimizing following objective.
\begin{theorem}[Informal]
\label{thm:objective}
Under certain regularity conditions, the solution to the optimization problem in \cref{eqn:joint_obj} can be written as follows:
% \chenlin{you can use resize box}
\begin{equation}
\label{eq:objective_simplified}
\resizebox{0.9\hsize}{!}{$
\begin{split}
    &\theta^{*} = \argmin_{\theta} \textrm{}
    \E_{p(t)}\E_{p_{t}(\rvx)}\E_{p({\rvv})}\bigg[ \\
    &\frac{1}{2}\lambda(t) \norm{\vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx]}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx] \rvv \\
    &+ \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta^{\textrm{joint}}(\rvx, t)[t] + \lambda'(t) \vs_\vtheta^{\textrm{joint}}(\rvx, t)[t]\bigg] \\
    &+ \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta^{\textrm{joint}}(\rvx, 0)[t]] - \E_{p_1(\rvx)}[\lambda(1) \vs_\vtheta^{\textrm{joint}}(\rvx, 1)[t]].
\end{split}
$}
\end{equation}
\end{theorem}
where $\rvv \sim p(\rvv) = \mathcal{N}(\bm{0}, \bm{I})$, $\vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx]$ denotes the data score component of $\vs_\vtheta^{\textrm{joint}}$, and $\vs_\vtheta^{\textrm{joint}}(\rvx, t)[t]$ denotes the time-score component of $\vs_\vtheta^{\textrm{joint}}$.
% \kristy{distribution of $\rvv$}
We defer the proof and detailed assumptions to Appendix~\ref{app-joint-proof}. In practice, the expectation in \cref{eq:objective_simplified} can be approximated via Monte Carlo sampling.
% This objective is beneficial in situations where we can only sample from 
% the intermediate densities $p_t(\rvx)$.
We can leverage DSM when
the data follows a known stochastic differential equation (SDE) and $p(\bx) = \mathcal{N}(\bm{0}, \bm{I})$
% For some choices of $p(\bx)$, 
% for example the standard normal Gaussian as in the MNIST energy-based modeling experiments (for specific choices of the forward SDE), 
% we can directly use DSM 
since the analytical form of $p_{t}(\bx)$ is tractable. 
% Similar to \cref{prop:time_objective}, the optimal score model trained via the joint objective satisfies $\vs_{\vtheta^*}^{\textrm{joint}}(\rvx, t) \approx [\nabla_\rvx \log p_{t}(\rvx); \dt \log p_{t}(\rvx)]$. This is because: 
% % $\vs_{\vtheta^*}^{\textrm{joint}}(\rvx, t) \approx \nabla_{[\rvx;t]} \log p(\rvx, t)$ and
% \begin{align*}
%     \nabla_\rvx \log p(\rvx, t) &= \nabla_\rvx \log p_{t}(\rvx) + \nabla_\rvx \log p(t) = \nabla_\rvx \log p_{t}(\rvx)\\
%     \dt \log p(\rvx, t) &= \dt \log p_{t}(\rvx) + \dt \log p(t) = \dt \log p_{t}(\rvx),
% \end{align*}
% since $p(t)$ does not depend on $\rvx$ and is a uniform distribution. 



==> sections/old/classification.tex <==
% \section{Classification}
% \kristy{TODO: There are a few questions that we should answer/threads to address}:
% \begin{enumerate}
%     \item We are effectively performing an infinite number of binary classification problems? Make the relationship between this and TRE clear (beyond density ratio estimation). Also think about weighting/noise schedules. But I guess the difference is that the time scores for the "intermediate classes" $t = y \in (0,1)$ are basically useless for classification (we'd just care about the final integrated value). Can we use these intermediate things in some other way beyond integrating? (say, if we wanted to do multi-class classification like in CIFAR-10)
%     \item Relationship between time score/joint training with NCE/conditional NCE? Because of the commonly known relationship between score matching + NCE, we could probably mention this in a sentence to make the connection
%     \item If we \textbf{purely} care about classification/density ratio estimation, not sure why we should care about estimating time scores rather than training a binary classifier
% \end{enumerate}

% \kristy{What we should clarify:}
% \begin{enumerate}
%     \item Is the gain coming from: (a) infinitely many interpolated distributions; OR (b) the score matching loss (vs. something like logistic loss); or both? \kristy{To address this question, we need to compare: (a) score-matching with finite $t$, (b) TRE with infinite waymarks (ODE solver baseline)}
%     \item A check that we can perform: if we take the density ratios from a trained TRE model, what happens if we plug it into the score matching loss? (discretized)
% \end{enumerate}

% We want to know if there is a way to train the continuous-time classifier with different scoring rules (logistic vs score matching). One thing to look into: if we take the logistic loss trained continuously (e.g. ODE), can we get back TRE?


==> sections/old/less_older_method.tex <==
\section{Time Score Matching via Infinitesimal Classification}
\label{time_training}
% We build some intuition about the time score in order to construct a suitable learning algorithm.
Intuitively, the time score can be approximated by the log density ratio between two intermediate distributions $p_t(\rvx)$ and $p_{t+\Delta t}(\rvx)$ with an infinitesimal gap ($\Delta t$):
% $\frac{\partial}{\partial t} \log p_t(\rvx) \approx \log p_{t+\Delta t}(\rvx)  - \log p_{t}(\rvx)$. 
$\frac{\partial}{\partial t} \log p_t(\rvx) \approx (\log p_{t+\Delta t}(\rvx)  - \log p_{t}(\rvx))/ \Delta t = (\log \frac{p_{t+\Delta t}(\rvx)}{p_{t}(\rvx)})/ \Delta t$.
Then analogous to TRE, we can construct an ``infinitesimal classification'' problem where the $t$-th intermediate classifier is tasked with distinguishing between samples from these two extremely close bridge distributions.
% Analogous to TRE, we can think of the time score as the $t$-th intermediate classifier distinguishing between two extremely close bridges, which we call ``infinitesimal classification''.

In fact, the following proposition formally states that the optimal form of this infinitesimal classifier 
is essentially given by the
% becomes an expression 
% \se{is essentially given by / can be easily obtained from the time score}
% of
% is parameterized by the 
time score $\dt \log p_t(\rvx)$.
\begin{proposition}
\label{prop:score_clf} When $T \rightarrow \infty$, the \se{is this the bayes-optimal?} optimal classifier between two adjacent bridge distributions $p_{t/T}(\rvx)$ and $p_{(t+1)/T}(\rvx)$ is: 
\begin{equation}
    % \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} O\left(\dt \log p_t(\rvx)\right).
    \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} \left(\dt \log p_t(\rvx)\right) \Delta t.
\end{equation}
\end{proposition}
\se{is this for any $t$?}
\se{double check the statemetn of this proposition. deltaT goes to zero in the limit}
where $\vh_{\vtheta^*}(\rvx, t) \in [0,1]$ is a conditional 
% \se{probabilistic?} 
probabilistic classifier  and $\Delta t = \frac{1}{T}$. 
% \kristy{is this accurate?}
% \ys{Need to mention somewhere that the big O is with respect to $\Delta t = 1/T$.}
% \se{big O notation doesn't make sense}

While the above result is instructive, it does not provide us with a practical algorithm for time score estimation---we have arrived at an impasse if we must somehow train an infinite number of such binary classifiers.
% \kristy{This is important because the identity in \cref{sum_to_integral} has conveniently converted the need to solve $T$ binary classification problems into one that requires the ability to estimate the time scores.}
% \se{give some intuition here. $\frac{\partial}{\partial t} \log p_t(\rvx) \approx \log p_{t+\delta_t}(\rvx)  - \log p_{t}(\rvx) = \log \frac{p_{t+\delta_t}(\rvx)} {p_{t}(\rvx)} $}
% This expression says that the form of the optimal infinitesimal classifier becomes an expression of how much each intermediate density is changing over time ($\dt \log p_t(\rvx)$). 
% In direct analogy to traditional data (Stein) scores $\nabla_\rvx \log p(\rvx)$, we name this quantity $\dt \log p_t(\rvx)$ the \emph{time score} function of $p_t(\rvx)$.
% The above proposition immediately suggests that we may be able to train a time score model \kristy{todo}$\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$. 
% To do so, 
Therefore,
we consider the limit of the binary cross-entropy loss function for the optimal infinitesimal classifier (\cref{prop:score_clf}) when $T\to \infty$.
% \ys{Missing a constant in the expression?} \kristy{which constant where?}
\begin{proposition}
\label{prop:opt_clf}
Let $\Delta t = 1/T$ and parameterize the binary classifier as $\vh_\vtheta(\rvx, t) = \frac{1}{2} + \frac{1}{4} \vs_\vtheta^{\textrm{time}}(\rvx, t)\Delta t$, where $\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$ denotes a time score model. Then from the binary cross-entropy objective:
\begin{equation}
% \label{eq:loss}
\resizebox{\linewidth}{!}{$
\begin{split}
    &\max_{\theta} \mathbb{E}_{p_{t}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t))] + \mathbb{E}_{p_{t+\Delta t}(\rvx)}[\log \vh_\vtheta(\rvx, t)]\\
    =& \max_{\theta} -\frac{1}{4} (\Delta t)^2 \mbb{E}_{p_t(\rvx)}\left[\left(\vs_\vtheta^{\textrm{time}}(\rvx, t) - \dt \log p_t(\rvx) \right)^2\right] + o((\Delta t)^2)
\end{split}
$}
\end{equation}
\end{proposition}
% \se{why is there a norm? these are scalars i think?}
% \se{there seems to be something wrong with the expreission (maybe the sign). it looks like you want to make the score model different from the true score in order to make the loss small?} \kristy{explicitly write max, we want to make this big}
We defer the proof to Appendix~\ref{pf-opt-clf}.
% With an interpolation mechanism in place, we 
% \kristy{transition} 
% \kristy{todo; clean up} 

\cref{prop:opt_clf} immediately suggests that a viable learning strategy will be to train a time score model $\vs_\vtheta^{\textrm{time}}(\rvx, t)$ to approximate the true time scores $\dt \log p_t(\rvx)$.
% strategy for learning the time scores will be to train a time score model $\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$.
We note that as the number of bridge distributions go to infinity,
% we increase the number of bridge distributions $T\to \infty$, 
we may drop some terms from the loss function as $\Delta t \to 0$.
\se{not sure i understand what this means?}
Therefore, we can simplify \cref{prop:opt_clf} into the following objective in order 
% \ys{As the number of bridge distributions increase to infinity, $T\to \infty$ and therefore $\Delta t \to 0$, in which case certain terms can be dropped in the loss function...} We can use the following expression
% We use this expression 
to train a time score model $s_\vtheta^{\textrm{time}}(\rvx, t)$:
\begin{equation}
\label{time_obj}
\resizebox{\linewidth}{!}{$
\begin{split}
        \mathcal{J_{\text{time}}(\theta)} &= \E_{p(t)}\E_{p_t(\rvx)}\bigg[\lambda(t) \left( \dt \log p_t(\rvx) - s_\vtheta^{\textrm{time}}(\rvx, t) \right)^2 \bigg]
\end{split}
$}
\end{equation}

\se{need to provide some guidance to the reader, the key issue is that the true score is unknown, so the objective cannot be evaluated let alone optimized}

\se{it's also not clear why we needed to talk about $\vh_{\vtheta^*}(\rvx, t)$, since then it's not used anymore. why is the score model also parameterized by theta? }

Then using integration by parts as in \citep{hyvarinen2005estimation}, we can show that this objective for learning $\dt \log p_t(\rvx)$ can be simplified to the following.

\begin{proposition}[Informal]
\label{prop:time_objective}
Under certain regularity conditions, the optimal solution $\theta^{*}$ of \cref{time_obj} is the same as the optimal solution of
\begin{equation}
\resizebox{\linewidth}{!}{$
\begin{split}
        &\mathcal{L_{\text{time}}(\theta)} = 2 \E_{q(\rvx)}[\lambda(0) s_\vtheta^{\textrm{time}}(\rvx, 0)] - 2\E_{p(\rvx)}[\lambda(1) s_\vtheta^{\textrm{time}}(\rvx, 1)] \\
    &+\E_{p(t)}\E_{p_t(\rvx)}\bigg[2 \lambda(t) \dt s_\vtheta^{\textrm{time}}(\rvx, t) + 2\lambda'(t) s_\vtheta^{\textrm{time}}(\rvx, t) + \lambda(t) s_\vtheta^{\textrm{time}}(\rvx, t)\bigg]
\end{split}
$}
\end{equation}
\end{proposition}
where the first two terms of \cref{prop:time_objective} denote the boundary conditions for $t=\{0,1\}$, and the expectations can be approximated via Monte Carlo. 
Our ability to estimate the objective via Monte Carlo samples makes training $\dreinf$
% the training procedure of $\dreinf$ 
much more efficient than TRE, which requires the explicit construction of $T$ additional batches per gradient step for all intermediate classifiers.
% intermediate classifier. \kristy{reword}
% \kristy{This gives us a nice objective that we can work with in practice.}
We defer the exact assumptions and proof to Appendix~\ref{pf-time-prop}, and provide pseudocode in Appendix~\ref{app-pseudo}.

The optimal time score model, denoted by $s_{\vtheta^\ast}^{\textrm{time}}(\rvx, t)$, satisfies $s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$. Therefore after training, the log-density-ratio can be estimated by:
\begin{equation}
    \label{eqn:dr1}
    \log r(\rvx) \approx \int_{1}^0 s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \ud t. 
\end{equation}
% \begin{align*}
%     \label{eqn:dr1}
%     \log r(\rvx) \approx \int_{1}^0 s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \ud t.
% \end{align*}
using any black-box numerical integrator as in \cref{sum_to_integral}.

\subsection{Joint Training Objective}
We can also incorporate
helpful auxiliary information from the data scores
into the training objective in \cref{time_obj}.
Specifically, we can define a vector-valued score model $\vs_\vtheta^{\textrm{joint}}(\rvx, t)$ and train it with a hybrid objective that seeks to \emph{jointly learn} $\nabla_{[\rvx; t]} \log p(\rvx, t)$:
\begin{equation}
\label{eqn:joint_obj}
\resizebox{\linewidth}{!}{$
        \mathcal{J_{\text{joint}}(\theta)} =
        \E_{p(t)}\E_{p_{t}(\rvx)}\left[ \frac{1}{2}\lambda(t)\norm{\nabla_{[\rvx; t]}\log p(\rvx, t) - \vs_\vtheta^{\textrm{joint}}(\rvx, t)}_2^2 \right].
$}
\end{equation}
We again note that the data score component in \cref{eqn:joint_obj} can be obtained by DSM \citep{vincent2011connection} or SSM \citep{song2020sliced}.
For the SSM variant, following \citep{hyvarinen2005estimation,song2020sliced} shows that optimizing \cref{eqn:joint_obj} is equivalent to the optimizing following objective.
\begin{theorem}[Informal]
\label{thm:objective}
Under certain regularity conditions, the solution to the optimization problem in \cref{eqn:joint_obj} can be written as follows:
% \chenlin{you can use resize box}
\begin{equation}
\label{eq:objective_simplified}
\resizebox{0.9\hsize}{!}{$
\begin{split}
    &\theta^{*} = \argmin_{\theta} \textrm{}
    \E_{p(t)}\E_{p_{t}(\rvx)}\E_{p({\rvv})}\bigg[ \\
    &\frac{1}{2}\lambda(t) \norm{\vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx]}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx] \rvv \\
    &+ \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta^{\textrm{joint}}(\rvx, t)[t] + \lambda'(t) \vs_\vtheta^{\textrm{joint}}(\rvx, t)[t]\bigg] \\
    &+ \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta^{\textrm{joint}}(\rvx, 0)[t]] - \E_{p_1(\rvx)}[\lambda(1) \vs_\vtheta^{\textrm{joint}}(\rvx, 1)[t]].
\end{split}
$}
\end{equation}
\end{theorem}
where $\rvv \sim p(\rvv) = \mathcal{N}(\bm{0}, \bm{I})$, $\vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx]$ denotes the data score component of $\vs_\vtheta^{\textrm{joint}}$, and $\vs_\vtheta^{\textrm{joint}}(\rvx, t)[t]$ denotes the time-score component of $\vs_\vtheta^{\textrm{joint}}$.
% \kristy{distribution of $\rvv$}
We defer the proof and detailed assumptions to Appendix~\ref{app-joint-proof}. In practice, the expectation in \cref{eq:objective_simplified} can be approximated via Monte Carlo sampling.
% This objective is beneficial in situations where we can only sample from 
% the intermediate densities $p_t(\rvx)$.
We can leverage DSM when
the data follows a known stochastic differential equation (SDE) and $p(\bx) = \mathcal{N}(\bm{0}, \bm{I})$
% For some choices of $p(\bx)$, 
% for example the standard normal Gaussian as in the MNIST energy-based modeling experiments (for specific choices of the forward SDE), 
% we can directly use DSM 
since the analytical form of $p_{t}(\bx)$ is tractable. 

Similar to \cref{prop:time_objective}, the optimal score model trained via the joint objective satisfies $\vs_{\vtheta^*}^{\textrm{joint}}(\rvx, t) \approx [\nabla_\rvx \log p_{t}(\rvx); \dt \log p_{t}(\rvx)]$. This is because: 
% $\vs_{\vtheta^*}^{\textrm{joint}}(\rvx, t) \approx \nabla_{[\rvx;t]} \log p(\rvx, t)$ and
\begin{align*}
    \nabla_\rvx \log p(\rvx, t) &= \nabla_\rvx \log p_{t}(\rvx) + \nabla_\rvx \log p(t) = \nabla_\rvx \log p_{t}(\rvx)\\
    \dt \log p(\rvx, t) &= \dt \log p_{t}(\rvx) + \dt \log p(t) = \dt \log p_{t}(\rvx),
\end{align*}
since $p(t)$ does not depend on $\rvx$ and is a uniform distribution. 

% \paragraph{Structured Interpolations via SDEs.} \kristy{take this out?}
% We briefly mention a special case of $\dreinf$'s interpolation mechanism where the analytical form of $p_t(\rvx)$ is tractable.
% One such example is a diffusion process, where the data generating process of $q(\rvx)$ is represented as a Markov chain that transforms a simple distribution $p_T(\rvx) \equiv p(\rvx)$
% into a target distribution $p_0(\rvx) \equiv q(\rvx)$ \citep{sohl2015deep,ho2020denoising,song2020score}. 
% This sequential procedure can be described as the solution to an It$\hat{\textrm{o}}$ stochastic differential equation (SDE):
% \[
% \dd\rvx = \bff(\rvx, t)\dd t + g(t)\dd \bw
% \]
% where $\bw$ represents Brownian motion, $\bff(\cdot,t): \mathbb{R}^D \rightarrow \mathbb{R}^D$ is the drift coefficient of $\rvx(t)$, and $g(\cdot): \mathbb{R} \rightarrow \mathbb{R}$ is the diffusion coefficient of $\rvx(t)$, where $\rvx(t) \sim p_t(\rvx)$. 
% % Intuitively, this equation governs how the intermediate density $p_t(\rvx)$ changes as a function of time and noise \citep{oksendal2003stochastic}, and induces a set of stochastic paths in distribution space $\{\rvx(t)\}_{t \in [0, 1]}$ across timesteps $t$ that connect the initial and target densities together. 

% For learning settings where our data follows a known SDE, 
% we can leverage the Fokker-Planck equation \citep{jordan1998variational,oksendal2003stochastic} to transform the data scores $\nabla_\rvx \log p_t(\rvx)$ into time scores \emph{without training an additional model}.
% The Fokker-Planck equation describes the time-evolution of the probability density $p_t(\rvx)$ associated with the SDE:
% \begin{equation}
% \label{fokker-planck}
% \resizebox{\linewidth}{!}{$
% \begin{split}
%     \frac{\partial}{\partial t}\log p_t(\rvx) &= -\nabla \cdot \bff - \bff \tran \nabla_\rvx \log p_t(\rvx) \\
%     &+ g^2(t) \left[ ||\nabla_\rvx \log p_t(\rvx) ||^2_2 + \textrm{tr}(\nabla_\rvx^2 \log p_t(\rvx)) \right]
% \end{split}
% $}
% \end{equation}
% where $\bff$ and $g$ are well-defined for tractable SDEs. 
% We can train a data score network $s_\vtheta^{\textrm{data}}(\rvx, t)$ to approximate $\nabla_\rvx \log p_t(\rvx)$ via sliced score matching (SSM) \citep{song2020sliced} or denoising score matching (DSM) \citep{vincent2011connection,song2019generative}. 

% % In addition, knowing that the data follows a tractable SDE allows us to leverage DSM in \cref{eqn:joint_obj}.
% % However, we can leverage DSM when
% % the SDE is known and $p(\bx) = \mathcal{N}(\bm{0}, \bm{I})$
% % % For some choices of $p(\bx)$, 
% % % for example the standard normal Gaussian as in the MNIST energy-based modeling experiments (for specific choices of the forward SDE), 
% % % we can directly use DSM 
% % since the analytical form of $p_{t}(\bx)$ is tractable. 


==> sections/old/method_v2.tex <==
\section{Time Score Matching via Infinitesimal Classification (v2)}
\label{time_training}
In fact, the following proposition formally states that the optimal form of this infinitesimal classifier 
is given by the time score $\dt \log p_t(\rvx)$.
\begin{proposition}
\label{prop:score_clf} When $T \rightarrow \infty$, the \se{is this the bayes-optimal?} optimal classifier between two adjacent bridge distributions $p_{t/T}(\rvx)$ and $p_{(t+1)/T}(\rvx)$ is: 
\begin{equation}
    % \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} O\left(\dt \log p_t(\rvx)\right).
    \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} \left(\dt \log p_t(\rvx)\right) \Delta t.
\end{equation}
\end{proposition}
\se{is this for any $t$?}
\se{double check the statemetn of this proposition. deltaT goes to zero in the limit}
where $\vh_{\vtheta^*}(\rvx, t) \in [0,1]$ is a conditional 
probabilistic classifier  and $\Delta t = \frac{1}{T}$. 
% \kristy{is this accurate?}
% \ys{Need to mention somewhere that the big O is with respect to $\Delta t = 1/T$.}
% \se{big O notation doesn't make sense}

While the above result is instructive, it does not provide us with a practical algorithm for time score estimation---we have arrived at an impasse if we must somehow train an infinite number of such binary classifiers.
% \kristy{This is important because the identity in \cref{sum_to_integral} has conveniently converted the need to solve $T$ binary classification problems into one that requires the ability to estimate the time scores.}
% \se{give some intuition here. $\frac{\partial}{\partial t} \log p_t(\rvx) \approx \log p_{t+\delta_t}(\rvx)  - \log p_{t}(\rvx) = \log \frac{p_{t+\delta_t}(\rvx)} {p_{t}(\rvx)} $}
% This expression says that the form of the optimal infinitesimal classifier becomes an expression of how much each intermediate density is changing over time ($\dt \log p_t(\rvx)$). 
% In direct analogy to traditional data (Stein) scores $\nabla_\rvx \log p(\rvx)$, we name this quantity $\dt \log p_t(\rvx)$ the \emph{time score} function of $p_t(\rvx)$.
% The above proposition immediately suggests that we may be able to train a time score model \kristy{todo}$\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$. 
% To do so, 
To tackle this challenge,
we consider the limit of the binary cross-entropy loss function for the optimal infinitesimal classifier (\cref{prop:score_clf}) when $T\to \infty$.
% \ys{Missing a constant in the expression?} \kristy{which constant where?}
\begin{proposition}
\label{prop:opt_clf}
Let $\Delta t = 1/T$ and parameterize the binary classifier as $\vh_\vtheta(\rvx, t) = \frac{1}{2} + \frac{1}{4} \vs_\vtheta^{\textrm{time}}(\rvx, t)\Delta t$, where $\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$ denotes a time score model. Then from the binary cross-entropy objective:
\begin{equation}
% \label{eq:loss}
\resizebox{\linewidth}{!}{$
\begin{split}
    &\max_{\theta} \mathbb{E}_{p_{t}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t))] + \mathbb{E}_{p_{t+\Delta t}(\rvx)}[\log \vh_\vtheta(\rvx, t)]\\
    =& \max_{\theta} -\frac{1}{4} (\Delta t)^2 \mbb{E}_{p_t(\rvx)}\left[\left(\vs_\vtheta^{\textrm{time}}(\rvx, t) - \dt \log p_t(\rvx) \right)^2\right] + o((\Delta t)^2)
\end{split}
$}
\end{equation}
\end{proposition}
% \se{why is there a norm? these are scalars i think?}
% \se{there seems to be something wrong with the expreission (maybe the sign). it looks like you want to make the score model different from the true score in order to make the loss small?} \kristy{explicitly write max, we want to make this big}
We defer the proof to Appendix~\ref{pf-opt-clf}.
% With an interpolation mechanism in place, we 
% \kristy{transition} 
% \kristy{todo; clean up} 

\cref{prop:opt_clf} immediately suggests that a viable learning strategy will be to train a time score model $\vs_\vtheta^{\textrm{time}}(\rvx, t)$ to approximate the true time scores $\dt \log p_t(\rvx)$.
\kristy{explicitly say that we can solve an ``infinite number of classification problems'' by time score matching}
% strategy for learning the time scores will be to train a time score model $\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$.
% We note that as the number of bridge distributions go to infinity,
% we increase the number of bridge distributions $T\to \infty$, 
% we may drop some terms from the loss function as $\Delta t \to 0$.
% \se{not sure i understand what this means?}
% Therefore, we can simplify \cref{prop:opt_clf} into the following objective in order
In fact, we can further simplify \cref{prop:opt_clf}
% \ys{As the number of bridge distributions increase to infinity, $T\to \infty$ and therefore $\Delta t \to 0$, in which case certain terms can be dropped in the loss function...} We can use the following expression
% We use this expression 
to obtain the following objective for training a time score model $s_\vtheta^{\textrm{time}}(\rvx, t)$:
\begin{equation}
\label{time_obj}
\resizebox{\linewidth}{!}{$
\begin{split}
        \mathcal{J_{\text{time}}(\theta)} &= \E_{p(t)}\E_{p_t(\rvx)}\bigg[\lambda(t) \left( \dt \log p_t(\rvx) - s_\vtheta^{\textrm{time}}(\rvx, t) \right)^2 \bigg]
\end{split}
$}
\end{equation}
% \se{need to provide some guidance to the reader, the key issue is that the true score is unknown, so the objective cannot be evaluated let alone optimized}
\se{it's also not clear why we needed to talk about $\vh_{\vtheta^*}(\rvx, t)$, since then it's not used anymore. why is the score model also parameterized by theta? }
Then using integration by parts as in \citep{hyvarinen2005estimation}, we can show that this objective for learning $\dt \log p_t(\rvx)$ can be simplified to the following.

\begin{proposition}[Informal]
\label{prop:time_objective}
Under certain regularity conditions, the optimal solution $\theta^{*}$ of \cref{time_obj} is the same as the optimal solution of
\begin{equation}
\resizebox{\linewidth}{!}{$
\begin{split}
        &\mathcal{L_{\text{time}}(\theta)} = 2 \E_{q(\rvx)}[\lambda(0) s_\vtheta^{\textrm{time}}(\rvx, 0)] - 2\E_{p(\rvx)}[\lambda(1) s_\vtheta^{\textrm{time}}(\rvx, 1)] \\
    &+\E_{p(t)}\E_{p_t(\rvx)}\bigg[2 \lambda(t) \dt s_\vtheta^{\textrm{time}}(\rvx, t) + 2\lambda'(t) s_\vtheta^{\textrm{time}}(\rvx, t) + \lambda(t) s_\vtheta^{\textrm{time}}(\rvx, t)\bigg]
\end{split}
$}
\end{equation}
\end{proposition}
where the first two terms of \cref{prop:time_objective} denote the boundary conditions for $t=\{0,1\}$, and the expectations can be approximated via Monte Carlo. 
Our ability to estimate the objective via Monte Carlo samples makes training $\dreinf$
% the training procedure of $\dreinf$ 
much more efficient than TRE, which requires the explicit construction of $T$ additional batches per gradient step for all intermediate classifiers.
% intermediate classifier. \kristy{reword}
% \kristy{This gives us a nice objective that we can work with in practice.}
We defer the exact assumptions and proof to Appendix~\ref{pf-time-prop}, and provide pseudocode in Appendix~\ref{app-pseudo}.

The optimal time score model, denoted by $s_{\vtheta^\ast}^{\textrm{time}}(\rvx, t)$, satisfies $s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$. Therefore after training, the log-density-ratio can be estimated by:
\begin{equation}
    \label{eqn:dr1}
    \log r(\rvx) \approx \int_{1}^0 s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \ud t. 
\end{equation}
% \begin{align*}
%     \label{eqn:dr1}
%     \log r(\rvx) \approx \int_{1}^0 s_{\vtheta^*}^{\textrm{time}}(\rvx, t) \ud t.
% \end{align*}
using any black-box numerical integrator as in \cref{sum_to_integral}.

\subsection{Joint Training Objective}
We can also incorporate
helpful auxiliary information from the data scores
into the training objective in \cref{time_obj}.
Specifically, we can define a vector-valued score model $\vs_\vtheta^{\textrm{joint}}(\rvx, t)$ and train it with a hybrid objective that seeks to \emph{jointly learn} $\nabla_{[\rvx; t]} \log p(\rvx, t)$:
\begin{equation}
\label{eqn:joint_obj}
\resizebox{\linewidth}{!}{$
        \mathcal{J_{\text{joint}}(\theta)} =
        \E_{p(t)}\E_{p_{t}(\rvx)}\left[ \frac{1}{2}\lambda(t)\norm{\nabla_{[\rvx; t]}\log p(\rvx, t) - \vs_\vtheta^{\textrm{joint}}(\rvx, t)}_2^2 \right].
$}
\end{equation}
We again note that the data score component in \cref{eqn:joint_obj} can be obtained by DSM \citep{vincent2011connection} or SSM \citep{song2020sliced}.
For the SSM variant, following \citep{hyvarinen2005estimation,song2020sliced} shows that optimizing \cref{eqn:joint_obj} is equivalent to the optimizing following objective.
\begin{theorem}[Informal]
\label{thm:objective}
Under certain regularity conditions, the solution to the optimization problem in \cref{eqn:joint_obj} can be written as follows:
% \chenlin{you can use resize box}
\begin{equation}
\label{eq:objective_simplified}
\resizebox{0.9\hsize}{!}{$
\begin{split}
    &\theta^{*} = \argmin_{\theta} \textrm{}
    \E_{p(t)}\E_{p_{t}(\rvx)}\E_{p({\rvv})}\bigg[ \\
    &\frac{1}{2}\lambda(t) \norm{\vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx]}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx] \rvv \\
    &+ \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta^{\textrm{joint}}(\rvx, t)[t] + \lambda'(t) \vs_\vtheta^{\textrm{joint}}(\rvx, t)[t]\bigg] \\
    &+ \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta^{\textrm{joint}}(\rvx, 0)[t]] - \E_{p_1(\rvx)}[\lambda(1) \vs_\vtheta^{\textrm{joint}}(\rvx, 1)[t]].
\end{split}
$}
\end{equation}
\end{theorem}
where $\rvv \sim p(\rvv) = \mathcal{N}(\bm{0}, \bm{I})$, $\vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx]$ denotes the data score component of $\vs_\vtheta^{\textrm{joint}}$, and $\vs_\vtheta^{\textrm{joint}}(\rvx, t)[t]$ denotes the time-score component of $\vs_\vtheta^{\textrm{joint}}$.
% \kristy{distribution of $\rvv$}
We defer the proof and detailed assumptions to Appendix~\ref{app-joint-proof}. In practice, the expectation in \cref{eq:objective_simplified} can be approximated via Monte Carlo sampling.
% This objective is beneficial in situations where we can only sample from 
% the intermediate densities $p_t(\rvx)$.
We can leverage DSM when
the data follows a known stochastic differential equation (SDE) and $p(\bx) = \mathcal{N}(\bm{0}, \bm{I})$
% For some choices of $p(\bx)$, 
% for example the standard normal Gaussian as in the MNIST energy-based modeling experiments (for specific choices of the forward SDE), 
% we can directly use DSM 
since the analytical form of $p_{t}(\bx)$ is tractable. 

Similar to \cref{prop:time_objective}, the optimal score model trained via the joint objective satisfies $\vs_{\vtheta^*}^{\textrm{joint}}(\rvx, t) \approx [\nabla_\rvx \log p_{t}(\rvx); \dt \log p_{t}(\rvx)]$. This is because: 
% $\vs_{\vtheta^*}^{\textrm{joint}}(\rvx, t) \approx \nabla_{[\rvx;t]} \log p(\rvx, t)$ and
\begin{align*}
    \nabla_\rvx \log p(\rvx, t) &= \nabla_\rvx \log p_{t}(\rvx) + \nabla_\rvx \log p(t) = \nabla_\rvx \log p_{t}(\rvx)\\
    \dt \log p(\rvx, t) &= \dt \log p_{t}(\rvx) + \dt \log p(t) = \dt \log p_{t}(\rvx),
\end{align*}
since $p(t)$ does not depend on $\rvx$ and is a uniform distribution. 

\subsection{Connections to Noise Contrastive Estimation (NCE)}
In fact, the following proposition formally states that the optimal form of this infinitesimal classifier 
is given by the time score $\dt \log p_t(\rvx)$.
\begin{proposition}
\label{prop:score_clf} When $T \rightarrow \infty$, the \se{is this the bayes-optimal?} optimal classifier between two adjacent bridge distributions $p_{t/T}(\rvx)$ and $p_{(t+1)/T}(\rvx)$ is: 
\begin{equation}
    % \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} O\left(\dt \log p_t(\rvx)\right).
    \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} \left(\dt \log p_t(\rvx)\right) \Delta t.
\end{equation}
\end{proposition}
\se{is this for any $t$?}
\se{double check the statemetn of this proposition. deltaT goes to zero in the limit}
where $\vh_{\vtheta^*}(\rvx, t) \in [0,1]$ is a conditional 
probabilistic classifier  and $\Delta t = \frac{1}{T}$. 
% \kristy{is this accurate?}
% \ys{Need to mention somewhere that the big O is with respect to $\Delta t = 1/T$.}
% \se{big O notation doesn't make sense}

While the above result is instructive, it does not provide us with a practical algorithm for time score estimation---we have arrived at an impasse if we must somehow train an infinite number of such binary classifiers.
% \kristy{This is important because the identity in \cref{sum_to_integral} has conveniently converted the need to solve $T$ binary classification problems into one that requires the ability to estimate the time scores.}
% \se{give some intuition here. $\frac{\partial}{\partial t} \log p_t(\rvx) \approx \log p_{t+\delta_t}(\rvx)  - \log p_{t}(\rvx) = \log \frac{p_{t+\delta_t}(\rvx)} {p_{t}(\rvx)} $}
% This expression says that the form of the optimal infinitesimal classifier becomes an expression of how much each intermediate density is changing over time ($\dt \log p_t(\rvx)$). 
% In direct analogy to traditional data (Stein) scores $\nabla_\rvx \log p(\rvx)$, we name this quantity $\dt \log p_t(\rvx)$ the \emph{time score} function of $p_t(\rvx)$.
% The above proposition immediately suggests that we may be able to train a time score model \kristy{todo}$\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$. 
% To do so, 
To tackle this challenge,
we consider the limit of the binary cross-entropy loss function for the optimal infinitesimal classifier (\cref{prop:score_clf}) when $T\to \infty$.
% \ys{Missing a constant in the expression?} \kristy{which constant where?}
\begin{proposition}
\label{prop:opt_clf}
Let $\Delta t = 1/T$ and parameterize the binary classifier as $\vh_\vtheta(\rvx, t) = \frac{1}{2} + \frac{1}{4} \vs_\vtheta^{\textrm{time}}(\rvx, t)\Delta t$, where $\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$ denotes a time score model. Then from the binary cross-entropy objective:
\begin{equation}
% \label{eq:loss}
\resizebox{\linewidth}{!}{$
\begin{split}
    &\max_{\theta} \mathbb{E}_{p_{t}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t))] + \mathbb{E}_{p_{t+\Delta t}(\rvx)}[\log \vh_\vtheta(\rvx, t)]\\
    =& \max_{\theta} -\frac{1}{4} (\Delta t)^2 \mbb{E}_{p_t(\rvx)}\left[\left(\vs_\vtheta^{\textrm{time}}(\rvx, t) - \dt \log p_t(\rvx) \right)^2\right] + o((\Delta t)^2)
\end{split}
$}
\end{equation}
\end{proposition}
% \se{why is there a norm? these are scalars i think?}
% \se{there seems to be something wrong with the expreission (maybe the sign). it looks like you want to make the score model different from the true score in order to make the loss small?} \kristy{explicitly write max, we want to make this big}
We defer the proof to Appendix~\ref{pf-opt-clf}.
% With an interpolation mechanism in place, we 
% \kristy{transition} 
% \kristy{todo; clean up} 








% \paragraph{Structured Interpolations via SDEs.} \kristy{take this out?}
% We briefly mention a special case of $\dreinf$'s interpolation mechanism where the analytical form of $p_t(\rvx)$ is tractable.
% One such example is a diffusion process, where the data generating process of $q(\rvx)$ is represented as a Markov chain that transforms a simple distribution $p_T(\rvx) \equiv p(\rvx)$
% into a target distribution $p_0(\rvx) \equiv q(\rvx)$ \citep{sohl2015deep,ho2020denoising,song2020score}. 
% This sequential procedure can be described as the solution to an It$\hat{\textrm{o}}$ stochastic differential equation (SDE):
% \[
% \dd\rvx = \bff(\rvx, t)\dd t + g(t)\dd \bw
% \]
% where $\bw$ represents Brownian motion, $\bff(\cdot,t): \mathbb{R}^D \rightarrow \mathbb{R}^D$ is the drift coefficient of $\rvx(t)$, and $g(\cdot): \mathbb{R} \rightarrow \mathbb{R}$ is the diffusion coefficient of $\rvx(t)$, where $\rvx(t) \sim p_t(\rvx)$. 
% % Intuitively, this equation governs how the intermediate density $p_t(\rvx)$ changes as a function of time and noise \citep{oksendal2003stochastic}, and induces a set of stochastic paths in distribution space $\{\rvx(t)\}_{t \in [0, 1]}$ across timesteps $t$ that connect the initial and target densities together. 

% For learning settings where our data follows a known SDE, 
% we can leverage the Fokker-Planck equation \citep{jordan1998variational,oksendal2003stochastic} to transform the data scores $\nabla_\rvx \log p_t(\rvx)$ into time scores \emph{without training an additional model}.
% The Fokker-Planck equation describes the time-evolution of the probability density $p_t(\rvx)$ associated with the SDE:
% \begin{equation}
% \label{fokker-planck}
% \resizebox{\linewidth}{!}{$
% \begin{split}
%     \frac{\partial}{\partial t}\log p_t(\rvx) &= -\nabla \cdot \bff - \bff \tran \nabla_\rvx \log p_t(\rvx) \\
%     &+ g^2(t) \left[ ||\nabla_\rvx \log p_t(\rvx) ||^2_2 + \textrm{tr}(\nabla_\rvx^2 \log p_t(\rvx)) \right]
% \end{split}
% $}
% \end{equation}
% where $\bff$ and $g$ are well-defined for tractable SDEs. 
% We can train a data score network $s_\vtheta^{\textrm{data}}(\rvx, t)$ to approximate $\nabla_\rvx \log p_t(\rvx)$ via sliced score matching (SSM) \citep{song2020sliced} or denoising score matching (DSM) \citep{vincent2011connection,song2019generative}. 

% % In addition, knowing that the data follows a tractable SDE allows us to leverage DSM in \cref{eqn:joint_obj}.
% % However, we can leverage DSM when
% % the SDE is known and $p(\bx) = \mathcal{N}(\bm{0}, \bm{I})$
% % % For some choices of $p(\bx)$, 
% % % for example the standard normal Gaussian as in the MNIST energy-based modeling experiments (for specific choices of the forward SDE), 
% % % we can directly use DSM 
% % since the analytical form of $p_{t}(\bx)$ is tractable. 


==> sections/old/old_method.tex <==
\section{Time Score Matching}
\label{method}
\subsection{Discrete Bridges to Continuous Paths}
\label{time_training}
To develop a more scalable alternative to \cref{eq:tre}, 
we propose to relax the number of bridges to infinity and consider a continuous \textit{path} of intermediate distributions connecting $p_0(\rvx)$ and $p_1(\rvx)$.
% \kristy{Concretely, we let a continuous value $t \in [0,1]$ index the intermediate sequences of probability distributions, and divide this range into $T > 0$ discrete steps. }
Then as shown in \citep{gelman1998simulating,owen2013monte,yao2020adaptive}, our telescoping sum is converted into an integral,
% in the limit of infinitely large $T$, 
where we integrate over the time scores $\dt \log p_t(\rvx)$ across the entire range of $t \in [0, 1]$:
\kristy{double check this, esp the last line}\chenlin{can we only keep 2 lines of the eq and move the details to appendix?}
\begin{align*}
    \log \frac{p_0(\rvx)}{p_1(\rvx)} &= \sum_{t=1}^{T} \log \left( \frac{p_{(t-1)/T}(\rvx)}{p_{t/T}(\rvx)} \right) \\
    &= \sum_{t=1}^T \log \left(1 + \frac{p_{(t-1)/T}(\rvx) - p_{t/T}(\rvx)}{p_{t/T}(\rvx)} \right)\\
    & \approx \lim_{T \rightarrow \infty} \frac{1}{T} \sum_{t=1}^T \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) \vert_{\lambda=t/T}\\
    &= \int_{1}^0 \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) d\lambda
\end{align*}
% \kristy{oooo}
% \begin{align*}
%     \log \frac{p_T(\rvx)}{p_0(\rvx)} &= \sum_{t=1}^T \log \left( \frac{p_{t/T}(\rvx)}{p_{(t-1)/T}(\rvx)} \right) \\
%     &= \sum_{t=1}^T \log \left(1 + \frac{p_{t/T}(\rvx) - p_{(t-1)/T}(\rvx)}{p_{(t-1)/T}(\rvx)} \right)\\
%     & \approx \lim_{T \rightarrow \infty} \frac{1}{T} \sum_{t=1}^T \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) \vert_{\lambda=(t-1)/T} = \int_{0}^1 \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) d\lambda
% \end{align*}
\chenlin{maybe define what T is?}
This idea is rooted in simulated annealing \citep{jarzynski1997nonequilibrium,neal2001annealed} and path sampling \citep{gelman1998simulating,blanchet2007path,yao2020adaptive}, which are advanced variance reduction techniques for importance sampling in the context of approximating intractable normalizing constants.

\kristy{TODO:
\begin{enumerate}
    \item definition 1
    \item time score
    \item how been used
    \item connect to data score
\end{enumerate}
}
% historically used for importance sampling and to approximate intractable normalizing constants in Markov Chain Monte Carlo (MCMC) simulations. \kristy{this might be redundant}
% We assume that there exists a path connecting the starting distribution $p_0(\rvx)$ to target distribution $p_T(\rvx)$. 
% Concretely, we let a continuous value $t \in [0,1]$ index the intermediate sequences of probability distributions, and divide this range into $T > 0$ discrete steps. Then, we can see that our telescoping sum is converted into an integral in the limit of infinitely large $T$, where we integrate over the time scores $\dt \log p_t(\rvx)$ across the entire range of $t$. 
% We include the proof sketch here for completeness \citep{gelman1998simulating,owen2013monte,yao2020adaptive}: \kristy{fix direction of T}
% % recover the well-known formula for path sampling
% \begin{align*}
%     \log \frac{p_T(\rvx)}{p_0(\rvx)} &= \sum_{t=1}^T \log \left( \frac{p_{t/T}(\rvx)}{p_{(t-1)/T}(\rvx)} \right) \\
%     &= \sum_{t=1}^T \log \left(1 + \frac{p_{t/T}(\rvx) - p_{(t-1)/T}(\rvx)}{p_{(t-1)/T}(\rvx)} \right)\\
%     & \approx \lim_{T \rightarrow \infty} \frac{1}{T} \sum_{t=1}^T \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) \vert_{\lambda=(t-1)/T} = \int_{0}^1 \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) d\lambda
% \end{align*}
% \kristy{todo} 
This identity has conveniently converted the need to solve $K$ binary classification problems into one that requires the ability to estimate the time scores $\dt \log p_t(\rvx)$.
% \kristy{Therefore, the approach hinges on the ability to learn the time scores $\dt \log p_t(\rvx)$.}
% This perspective allows us to directly leverage recent advances in score-based generative modeling in order to learn the $\frac{\partial}{\partial t} \log p_t(\rvx)$, which we denote as the \textit{time scores}. 
% \kristy{maybe we want to talk about how this quantity might be hard to estimate naively.}
% where in the 4th line we have used a first-order Taylor expansion around $0$ and in the 5th line we use the definition of the derivative.

\subsection{Time-wise Score Estimation}
There exist various ways to estimate the time scores from data, which we describe in our time score matching framework.
% brings us to the core technical contribution of this work. 
Our framework is fully general, in that we do not require the data generating process to follow a prescribed SDE or diffusion process;
% a prescribed form of the SDE or even require the data generating process to follow a particular diffusion process; 
our method only requires that we be able to sample from all the distributions along the spectrum of $q(\rvx)$ and $p(\rvx)$. 

\paragraph{Known SDE/Diffusion process.} For learning settings where our data follows a known SDE, 
% \kristy{is this accurate?}\ys{seems right to me}, 
we can leverage the Fokker-Planck equation \citep{jordan1998variational,oksendal2003stochastic} to transform the data scores $\nabla_\rvx \log p_t(\rvx)$ into time scores \emph{without training an additional model}.
The Fokker-Planck equation describes the time-evolution of the probability density $p_t(\rvx)$ associated with the SDE:
% , and can be used to obtain an estimate of the time scores via a transformation of the data scores $\nabla_\rvx \log p_t(\rvx)$:
\begin{equation}
\label{fokker-planck}
\resizebox{\linewidth}{!}{
\begin{split}
    \frac{\partial}{\partial t}\log p_t(\rvx) &= -\nabla \cdot \bff - \bff \tran \nabla_\rvx \log p_t(\rvx) \\
    &+ g^2(t) \left[ ||\nabla_\rvx \log p_t(\rvx) ||^2_2 + \textrm{tr}(\nabla_\rvx^2 \log p_t(\rvx)) \right]
\end{split}
}
\end{equation}
% \chenlin{should it be
% \begin{equation}
%     \frac{\partial}{\partial t}\log p_t(\rvx) = -\nabla \cdot \bff - \bff \tran \nabla_\rvx \log p_t(\rvx) + \frac{g^2(t)}{2} \left[ ||\nabla_\rvx \log p_t(\rvx) ||^2_2 + \textrm{sum}(\nabla_\rvx^2 \log p_t(\rvx)) \right]
% \end{equation}
% divided by $2$ can be removed depending on parameterization.
% }
% \chenlin{can the score on t be derived from data score? yes, but it involves the trace term, which is estimated by hutchison's trace estimator since otherwise it would be too expensive}
where $\bff$ and $g(\cdot)$ are well-defined for SDEs such as the Variance Preserving SDE (VPSDE) in diffusion probabilistic models.
With recent advances in score-based generative modelsg, we can train a data score network $s_\vtheta(\rvx, t)$ to approximate $\nabla_\rvx \log p_t(\rvx)$ with denoising score matching (DSM) \citep{vincent2011connection} or sliced score matching (SSM) \citep{song2020sliced}. 
% For SDEs such as the Variance Preserving SDE (VPSDE), these quantities are well-defined, and we can use the output of a trained score network $s_\vtheta(\rvx, t)$ to approximate $\nabla_\rvx \log p_t(\rvx)$. 
The $\nabla \cdot \bff$ term can be estimated efficiently via the Skilling-Hutchinson trace estimator \citep{skilling1989eigenvalues,hutchinson1989stochastic}.
% For computational efficiency, we can leverage the Skilling-Hutchinson trace estimator \citep{skilling1989eigenvalues,hutchinson1989stochastic} to compute $\nabla \cdot \bff$.
% \kristy{todo} The data score $\nabla_\rvx \log p_t(\rvx)$ can be obtained by leveraging recent advances from score-based generative models, either via 
% We note that the quantity $\nabla_\rvx \log p_t(\rvx)$ can be obtained by training a data score network either via 
% denoising score matching (DSM) \citep{vincent2011connection} or sliced score matching (SSM) \citep{song2020sliced}. 

\paragraph{Unknown SDE.} 
% In many practical scenarios where we do not know the data distribution's underlying SDE,
Although many practical scenarios do not grant us access to the data distribution's underlying SDE,
% \chenlin{what does data's underlying SDE mean?}
there are many ways to specify the intermediate distributions $p_{t}(\rvx)$ given $p(\rvx)$ and $q(\rvx)$.
% However, many practical scenarios do not have grant us access to the underlying SDE. 
% Our framework is fully general, in the sense that we do not require a prescribed form of the SDE or even require the data generating process to follow a particular diffusion process; our method only requires that we be able to sample from all the distributions along the spectrum of $p_1(\rvx)$ and $p_0(\rvx)$. 
% , or we only have access to \textit{samples} of the intermediate distributions $\log p_t(\rvx)$, or we do not have access to the $\nabla_\rvx \log p_t(\rvx)$. \kristy{clean this up}. \kristy{transition or take out} 
% Note that there are many ways to specify $p_{t}(\rvx)$ given $p(\rvx)$ and $q(\rvx)$ even without specifying an SDE. 
For example, we can define a sample from $p_{t}(\rvx)$ as $\rvx(t) := \sqrt{1-\alpha(t)^2} \rvx + \alpha(t) \rvy$, where $\rvx \sim q$, $\rvy \sim p$, and $\alpha: [0,1] \to \R^+$ is a positive function that satisfies $\alpha(0) = 0$ and $\alpha(1) = 1$. 
% Alternatively, the $p_t(\rvx)$ may be given by a pre-specified SDE. 
% Our framework is fully general, in the sense that we do not require a prescribed form of the SDE or even require the data generating process to follow a particular diffusion process.
% We only require that we be able to sample from all the distributions along the spectrum of $p_1(\rvx)$ and $p_0(\rvx)$.
% We note that in the log probability density $\log p_t(\rvx)$, we may compute the scores with respect to $t$, which we call the \textit{time score} $\frac{\partial}{\partial t} \log p_t(\rvx)$. Intuitively, the time score measures how much the density is changing across time, or how much the intermediate distribution is changing as we transport our samples $\rvx$ from the starting distribution $p_0(\rvx)$ to the target distribution $p_T(\rvx)$. 
% Intuition: want to bridge the gap between $p_0(\rvx)$ and $p_T(\rvx)$. Can do so with intermediate distributions (samples from them), and will get better estimates with more intermediate distributions (but this leads to a lot more compute). 
% \begin{enumerate}
%     \item Would be good to give some intuition about the distinction between $\frac{\partial}{\partial t} \log p_t(\rvx)$ and data scores $\nabla_x \log p_t(\rvx)$. Concretely answer: what does a "time-score" represent?
%     \item Maybe via a toy example? (the 1-D) setting
%     \item Could talk about the relationship between the data scores and the time scores (e.g. Fokker-Planck for DDPM)
%     \item conservative vector field stuff? (re: path integrals?)
% \end{enumerate}
% \kristy{This subsection should make it clear as to why considering the time scores of the data is a good idea}
% \subsection{Time-wise Score Matching}
% In order to estimate $\frac{\partial \log p_{t}(\rvx)}{\partial t}$, 
In such a setting, we must turn to \textit{learning} the time scores. With an interpolation mechanism in place, we propose to train a score model $s_\vtheta(\rvx, t)$ with the following score matching objective:
\begin{equation}
\label{time_obj}
\resizebox{\linewidth}{!}{
\begin{split}
        \mathcal{J_{\text{time}}(\theta)} &= \E_{t\sim \mcal{U}[0,1]}\E_{\rvx \sim p_{t}(\rvx)}\bigg[\lambda(t) \left( \frac{\partial \log p_{t}(\rvx)}{\partial t} - s_\vtheta(\rvx, t) \right)^2 \bigg]
\end{split}
}
\end{equation}
\chenlin{$s_\vtheta(\rvx, t)$ is time score or data score? have you introduced this notation?}
\chenlin{consider writing is as
\begin{equation}
\label{time_obj}
\resizebox{\linewidth}{!}{
\begin{split}
        \mathcal{J_{\text{time}}(\theta)} &= \E_{t}\E_{\rvx }\bigg[\lambda(t) \left( \frac{\partial \log p_{t}(\rvx)}{\partial t} - s_\vtheta(\rvx, t) \right)^2 \bigg],
\end{split}
}
\end{equation}
$t\sim \mcal{U}, \rvx \sim p_{t}(\rvx)$
}
Using integration by parts, we can show that 
% optimizing \cref{time_obj} is equivalent to optimizing 
% \begin{equation}
% \resizebox{\linewidth}{!}{
% \begin{split}
%         &\mathcal{L_{\text{time}}(\theta)} = 2 \E_q[\lambda(0) s_\vtheta(\rvx, 0)] - 2\E_p[\lambda(1) s_\vtheta(\rvx, 1)] \\
%     &+\E_{t\sim \mcal{U}[0,1]}\E_{\rvx \sim p_{t}(\rvx)}\bigg[2 \lambda(t) \frac{\partial s_\vtheta(\rvx, t)}{\partial t} + 2\lambda'(t) s_\vtheta(\rvx, t) + \lambda(t) s_\vtheta^2(\rvx, t)\bigg]
% \end{split}
% }
% \end{equation}

% in the following proposition that the time-wise scoring matching objective in \cref{time_obj} is equivalent to the expression below:
% \begin{theorem}[Informal]
% \label{thm:objective}
% Under certain regularity conditions, the solution to the optimization problem in \cref{eqn:joint_obj} can be written as follows:
% % \chenlin{you can use resize box}
% \begin{equation}
% \label{eq:objective_simplified}
% % \resizebox{0.9\hsize}{!}{
% \begin{split}
%     &\theta^{*} = \argmin_{\theta} \textrm{}
%     \E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\E_{\rvv \sim \mcal{N}(\bm{0}, \mI)}\bigg[ \\
%     &\frac{1}{2}\lambda(t) \norm{\vs_\vtheta(\rvx, t)}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta(\rvx, t) \rvv \\
%     &+ \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta(\rvx, t)[t] + \lambda'(t) \vs_\vtheta(\rvx, t)[t]\bigg] \\
%     &+ \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta(\rvx, 0)[t]] - \E_{p_1(\rvx)}[\lambda(1) \vs_\vtheta(\rvx, 1)[t].
% \end{split}
% % }
% \end{equation}
% \end{theorem}
\begin{proposition}[Informal]
\label{prop:time_objective}
Under certain regularity conditions, \kristy{TODO}
optimizing \cref{time_obj} is equivalent to optimizing 
\begin{equation}
\resizebox{\linewidth}{!}{
\begin{split}
        &\mathcal{L_{\text{time}}(\theta)} = 2 \E_q[\lambda(0) s_\vtheta(\rvx, 0)] - 2\E_p[\lambda(1) s_\vtheta(\rvx, 1)] \\
    &+\E_{t\sim \mcal{U}[0,1]}\E_{\rvx \sim p_{t}(\rvx)}\bigg[2 \lambda(t) \frac{\partial s_\vtheta(\rvx, t)}{\partial t} + 2\lambda'(t) s_\vtheta(\rvx, t) + \lambda(t) s_\vtheta^2(\rvx, t)\bigg]
\end{split}
}
\end{equation}
% \chenlin{can you remove the const term? since it does not affect optimization}
\end{proposition}
% \allowdisplaybreaks
% \begin{equation}
% \label{time_obj}
% \resizebox{\linewidth}{!}{
% \begin{split}
%         \mathcal{L_{\text{time}}(\theta)} &= \E_{t\sim \mcal{U}[0,1]}\E_{\rvx \sim p_{t}(\rvx)}\bigg[\lambda(t) \left( \frac{\partial \log p_{t}(\rvx)}{\partial t} - s_\vtheta(\rvx, t) \right)^2 \bigg] \\
%     &= 2 \E_q[\lambda(0) s_\vtheta(\rvx, 0)] - 2\E_p[\lambda(1) s_\vtheta(\rvx, 1)]\\
%     &+\E_{t\sim \mcal{U}[0,1]}\E_{\rvx \sim p_{t}(\rvx)}\bigg[2 \lambda(t) \frac{\partial s_\vtheta(\rvx, t)}{\partial t} + 2\lambda'(t) s_\vtheta(\rvx, t) \\
%     &+ \lambda(t) s_\vtheta^2(\rvx, t)\bigg] + \textnormal{const.}
% \end{split}
% }
% \end{equation}
where the first two terms of \cref{prop:time_objective} denote the boundary conditions for $t=\{0,1\}$, and the expectations can be approximated via Monte Carlo sampling. 
We defer the proof to Appendix~\ref{pf-time-prop}.

% \chenlin{do we plan to mention how we perform reweighting somewhere?}

\subsection{Network Architecture and Variance Reduction via Importance Weighting} 
\chenlin{this section is talking about empirical implementation, not technical method. so i think it could be combined with pathwise method section 4.1. and you can move section 3.4 and section 4.2 (with the training objective) before this section, 3.3 and 4.1 in a later section}\chenlin{we can talk about technical method first, and them empirical implementation}
\label{impl-design}
In our preliminary experiments, we found that a naive implementation of \cref{time_obj} led to unstable training due to the high variance in the objective across the different timescales $t$.
This finding is in accordance with recent work on diffusion probabilistic models \citep{nichol2021improved,kingma2021variational,song2021maximum}, which emphasize the critical role of applying the proper weighting function $\lambda(t)$ rather than randomly sampling $t \sim \mathcal{U}[0,1]$.
% as well as finding the proper correspondence to maximum likelihood training \kristy{clean up}. 
This problem is also exacerbated by the fact that our training objective requires backpropagating through the score network $s_\vtheta(\rvx, t)$ with respect to $t$, which can cause training to diverge or progress extremely slowly for certain design choices.
% choices of the model architecture.
% Specifically, backpropagating through the time score network with the term $\dt s_\vtheta(\rvx, t)$ required care. 

% \kristy{Maybe note that $\lambda(t)$ is dependent on the SDE and interpolation scheme? so hard to learn the function directly?} 
\paragraph{Selecting weighting schemes} Drawing inspiration from \citep{nichol2021improved}, we learn an importance weighting scheme of the distribution over timescales $p(t)$.
We maintain a history buffer of the $B$ most recent loss values (excluding the boundary conditions which are constant w.r.t. $t$),
and use this buffer to approximate a weighting function $\alpha(t) \approx \lambda(t): [0,1] \rightarrow \mathbb{R}_+$ designed to reduce the variance of the loss.
% by maintaining a loss history of buffer size $B$.
Specifically, we perform a polynomial interpolation for every new minibatch of $t$ sampled from $\mathcal{U}[0,1]$ during training.
% Concretely, we keep track of the $B$ most recent loss values (excluding the boundary conditions which are constant w.r.t. $t$), and use this buffer to fit a ridge regression model for approximating the proper weighting function $w(t) \approx \lambda(t)$.
% Once this model has been learned, we perform a polynomial interpolation for each minibatch of $t \sim \mathcal{U}[0,1]$
% (\kristy{todo: ridge regression with polynomial features}) 
% to learn a proper weighting function $w(t) \approx \lambda(t)$ designed 
% to reduce the variance in the loss. 
% across $t$. 
The weights obtained from this weighting function is then used to importance weight the expectation in \cref{time_obj}. 

\paragraph{Selecting embeddings} When designing the time score network architecture, we found that both sinusoidal positional embeddings \citep{ho2020denoising,song2020denoising} and Fourier embeddings \citep{tancik2020fourier,song2020score,kingma2021variational} commonly used in the literature led to training instabilities when computing $\dt \vs_{\vtheta}(\rvx, t)$. 
We hypothesize that this is due to the periodic nature of the sine and cosine functions, causing gradient information with respect to $t$ to oscillate during training.
Therefore, we fed the time-conditioning signal into a single hidden-layer Multilayer Perception (MLP) with Tanh activation functions prior to combining it with the input features.
% combined the time-conditioning signal with the input features via a simple 3-layer Multilayer Perceptron (MLP), where we used an embedding size of 256 and Tanh activation functions. 
We composed this time embedding module with a convolutional U-Net architecture \citep{ronneberger2015u}, which gave us the biggest performance boost, for our experiments.
We refer the reader to Appendix~\ref{app:loss_history} for additional details.
% We found this variance reduction technique to be very important for the energy-based modeling experiments on MNIST. 


% \subsection{Density Ratio Estimation with Time Scores}
\subsection{Leveraging the ODE Solver for Density Ratio Estimation}
After training a time-conditioned score network with \cref{time_obj}, it is straightforward to see that $\log r(\rvx)$ can be obtained via the following formula:
% Given $\{p_{t}(\rvx)\}_{t=0}^T$, a continuum of intermediate distributions between $p$ and $q$, we can compute $r(\rvx)$ via the following formula:
\begin{align}
    \log r(\rvx) = \int_{1}^0 \frac{\partial \log p_{t}(\rvx)}{\partial t} \ud t \approx \int_{1}^0 \vs_{\vtheta}(\rvx, t) \ud t. 
    \label{eqn:dr1}
\end{align}
% For the joint training objective, \cref{eqn:dr1} only requires the last dimension (time dimension) of $\vs_\vtheta(\rvx, t)[t]$.
The integration over all intermediate time scores in \cref{eqn:dr1} can be computed
% This simple variant only requires a trained time-score network, as well as a way to perform numerical integration 
using any existing numerical ODE solver. 
In this way, the ODE solver determines the timesteps $t$ we should query along the trajectory as we obtain our density ratio estimates, which eliminates the need to hand-tune $T$ as in \cref{eq:tre}.
% Then, we can integrate over all the intermediate time scores to obtain our density ratio estimates, 
% with the ODE solver dictating the timesteps $t$ we should query along the trajectory. 
% We found empirically that omitting these boundary terms led to poor performance of the score network.
% The optimal score model, denoted by $s_{\vtheta^\ast}(\rvx, t)$, satisfies $s_{\vtheta^*}(\rvx, t) \approx \frac{\partial \log p_{t}(\rvx)}{\partial t}$. 
Figure~\ref{fig:2d_exp}(d) demonstrates that a time-conditioned score network in this way indeed improves over specifying a finite number of intermediate distributions as in TRE.
% After training a time-conditioned score network in this way, we can see in Figure~\ref{fig:2d_exp}(d) that the model indeed improves over specifying only a finite number of intermediate distributions. \kristy{TODO}


==> sections/old/old_ratios.tex <==
\section{Pathwise Density Ratio Estimation}
% \kristy{THIS ENTIRE SECTION NEEDS TO BE FIXED}
\subsection{Incorporating Auxiliary Information via Data Scores}
\label{joint_training}
\kristy{THIS SECTION NEEDS FIXING}
% \chenlin{think about the design of optimal path that connects x to y. what is its connection to TRE with an infinitely amount of telescoping terms, and a classifier depending on t?}
Despite the improvements from leveraging an infinite number of intermediate distributions, 
% the na\"{i}ve application of \cref{eqn:dr1} 
\cref{eqn:dr1} does not address the fact that a fixed $\rvx$ typically cannot lie in the high data density regions of $p_{t}(\rvx)$ for all $t$ in practice.
% is unlikely to be successful in real-world settings because a fixed $\rvx$ typically cannot lie in the high data density regions of $p_{t}(\rvx)$ for all $t$
% \chenlin{it seems "contradictory" to your motivation? you mentioned we propose a method that can solve the density estimation issue, then you said our proposed method is unlikely to work? maybe you can say the pathwise method works better than the naive one instead of saying the naive one cannot work}. 
% However \kristy{TODO: as can be seen from the intuitive example hopefully??}, the na\"{i}ve application of \cref{eqn:dr1} is unlikely to be successful, because a fixed $\rvx$ typically cannot lie in the high data density regions of $p_{t}(\rvx)$ for all $t \in [0,1]$. 
We demonstrate this point in Figure~\ref{fig:bridge_err_simple_paths}(a), which illustrates the behavior of TRE(4)'s\chenlin{why do we have tre here?} (Section~\ref{bin_clf}) final intermediate classifier on various test points.
\kristy{TODO!!}
% by examining the behavior of a pre-trained TRE model's last intermediate classifier 
% This is demonstrated by a closer examination of a pre-trained TRE model, where its last intermediate classifier is shown as an illustrative example in 
% the last intermediate classifier in a pre-trained TRE model, as shown in 
% Figure~\ref{fig:bridge_err_simple_paths}(a). 
Recall that this particular classifier is trained to distinguish
% corresponds to solving the task of distinguishing 
between samples from $p_{(T-1)/T}(\rvx) = \mcal{N}\left(\sqrt{1-(\frac{T-1}{T})^2}\cdot \bm{4}, \mI \right)$ and $p_1(\rvx) = \mcal{N}(\bm{0}, \mI)$. 
As we evaluate this classifier on samples from $p_1(\rvx)$ and increasingly shift their means further away from 0, 
% $\rvx \sim \mathcal{N}([0, $
% points drawn from isotropic Gaussians whose means are further away from 0, 
% As $\rvx \sim p(\rvx)$ is shifted further away from an isotropic Gaussian of mean 0, 
the mean squared error between the true log ratio $\log r_3(\rvx)$\chenlin{have you defined what $r_3$ is?} and the estimated log ratio increases. 
This is particularly problematic, as it suggests that the density ratio estimates for samples drawn from $p_0(\rvx)$ are inaccurate.
% samples $\rvx \sim q(\rvx)$ correspond to a shift of 4. 
Therefore, this mismatch between train and test conditions leaves more room for improvement.
% Thus even if the intermediate bridges are more accurate for their interpolated samples during training, they are still inaccurate for points that lie in regions of low density \emph{at test time}.
% We observe this phenomenon across all intermediate classifiers trained via TRE. 

\begin{figure*}[!t]
    \centering
        \subfigure[MSE of TRE's intermediate classifier]{\includegraphics[width=.4\textwidth]{figures/bridge_3_errors.png}}
        \subfigure[A line path bridging high-density regions of $q(\rvx)$ and $p(\rvx)$]{\includegraphics[width=.4\textwidth]{figures/paths/line_path.png}}
    \caption{(a) Illustration of a failure mode of TRE. As the evaluation point is moved further away from samples drawn from the corresponding bridge density, the accuracy of the estimated likelihood ratio by the intermediate classifier degrades.
    (b) An example of the simple line path $\rvy(t) = \rvx + t \cdot (\rvz - \rvx)$ bridging the high-density regions of $q(\rvx)$ and $p(\rvx)$, where $\rvz$ is fixed to be the mean of $p(\rvx)$.}
    \label{fig:bridge_err_simple_paths}
\end{figure*}
% \kristy{todo} illustrative example on last bridge of TRE classifier.
% \begin{figure}[!ht]
%     \centering
%         \includegraphics[width=.55\textwidth]{figures/bridge_3_errors.png}
%     \caption{\kristy{todo} As x is shifted further from the distribution from where it was trained on, the mean squared error between the true log ratio for that intermediate density and the estimated log ratio increases.}
%     \label{fig:bridge_err}
% \end{figure}

To mitigate this difficulty, we propose to connect $\rvx$ in the high data density region of $p_0(\rvx)$ to $\rvy$ in the high data density region of $p_1(\rvx)$. 
To do so, we first prescribe a trajectory according to an ODE:
\begin{align*}
    \begin{cases}
    \rvy'(t) = \vf(\rvy, t)\\
    \rvy(0) = \rvx.
    \end{cases}
\end{align*}
\chenlin{have we defined what $f$ is?}
A simple example of such a path is the line $\rvy(t) = \rvx + t \cdot (\rvz - \rvx)$ as shown in Figure~\ref{fig:bridge_err_simple_paths}(b), where $\rvy'(t) = (\rvz - \rvx)$. 
A reasonable choice for $\rvz$ in this case is the mean of $p(\rvx)$, but it can also be obtained by sampling from $p(\rvx)$. 
We note that this is but one particular choice out of several for the path connecting $p(\rvx)$ and $q(\rvx)$ \citep{gelman1998simulating}. 
Although this pathwise density ratio estimation approach theoretically yields the same density ratio as computed directly from the time scores, we empirically verify that it gives more accurate results in practice in Figure~\ref{fig:2d_exp_shift1}. 

Using this path, the difference between $\log q(\rvx)$ and $\log p(\rvy)$ can be obtained by integration
\begin{align*}
    \log q(\rvx) - \log p(\rvy) = \int_1^0 \frac{\partial \log p_t(\rvy(t))}{\partial t} + \vf(\rvy(t), t)\tran \nabla_\rvx \log p_t(\rvy(t)) \ud t.
\end{align*}
Finally, we can compute the density ratio via the following expression:
\begin{equation}
\label{eq:pathwise}
    \begin{split}
            r(\rvx) &= \log q(\rvx) - \log p(\rvy) + \log p(\rvy) - \log p(\rvx) \\
    &= \int_1^0 \frac{\partial \log p_t(\rvy(t))}{\partial t} + \vf(\rvy(t), t)\tran \nabla_\rvx \log p_t(\rvy(t)) \ud t + \int_1^0 \nabla_\rvx \log q(\rvy + t(\rvx - \rvy))\tran (\rvx - \rvy) \ud t.
    \end{split}
\end{equation}
% \begin{equation}
% \label{eq:pathwise}
%     \begin{split}
%             r(\rvx) &= \log p(\rvy) - \log p(\rvx) + \log q(\rvx) - \log p(\rvy) \\
%     &= \int_1^0 \nabla_\rvx \log q(\rvy + t(\rvx - \rvy))\tran (\rvx - \rvy) \ud t + \int_1^0 \frac{\partial \log p_t(\rvy(t))}{\partial t} + \vf(\rvy(t), t)\tran \nabla_\rvx \log p_t(\rvy(t)) \ud t.
%     \end{split}
% \end{equation}

% Using this path, the difference between $\log p(\rvx)$ and $\log q(\rvy)$ can be obtained by integration
% \begin{align*}
%     \log q(\rvy) - \log p(\rvx) = \int_0^1 \frac{\partial \log p_t(\rvy(t))}{\partial t} + \vf(\rvy(t), t)\tran \nabla_\rvx \log p_t(\rvy(t)) \ud t.
% \end{align*}
% Finally, we can compute the density ratio via the following expression: \kristy{TODO: NOTATION}
% \begin{equation}
% \label{eq:pathwise}
%     \begin{split}
%             r(\rvx) &= \log q(\rvx) - \log q(\rvy) + \log q(\rvy) - \log p(\rvx) \\
%     &= \int_0^1 \nabla_\rvx \log q(\rvy + t(\rvx - \rvy))\tran (\rvx - \rvy) \ud t + \int_0^1 \frac{\partial \log p_t(\rvy(t))}{\partial t} + \vf(\rvy(t), t)\tran \nabla_\rvx \log p_t(\rvy(t)) \ud t.
%     \end{split}
% \end{equation}
% This trajectory connects $\rvx$ in the high data density region of $p_0(\rvx)$ to $\rvy$ in the high data density region of $p_1(\rvx)$. 

% \chenlin{is there a notation clash in $ \nabla_\rvx \log q(\rvy + t(\rvx - \rvy))\tran$, $\nabla_\rvx$ }
% \chenlin{is it true that $ \nabla_\rvx \log q(\rvy + t(\rvx - \rvy))\tran$ the derivative is w.r.t. to $\rvx$
% or the entire term in the parenthesis? it seems to cause an extra $t$? 
% will double check} 


% \kristy{The takeaway here is that this score-based framework makes it very easy to incorporate auxiliary information when learning these densities!}




\subsection{Joint Training Objective}
%We know that the optimal score-based model satisfies $\vs_{\vtheta^*}(\rvx, t) \approx [\nabla_\rvx \log p_{t}(\rvx); \partial_t \log p_{t}(\rvx)]$. Therefore, for the expression $\log q(\rvy) - \log p(\rvx)$, we have:
% \begin{align*}
%     \log q(\rvy) - \log p(\rvx) \approx \int_0^T \vs_{\vtheta^*}(\rvy(t), t)[t] + f(\rvy(t),t)
%     \tran \vs_{\vtheta^*}(\rvy(t), t)[\rvx] \ud t
% \end{align*}
% which means for the final density ratio estimate we have:
% \begin{equation}
%     \begin{split}
%   r(\rvx) &\approx \int_0^1 \nabla_\rvx \log q(\rvy + t(\rvx - \rvy))\tran (\rvx - \rvy) \ud t + \int_0^T \vs_{\vtheta^*}(\rvy(t), t)[t] + f(\rvy(t),t)\tran \vs_{\vtheta^*}(\rvy(t), t)[\rvx] \ud t \\
%   &\approx \int_0^1 \vs_{\vtheta^*}(\rvy(T) + t(\rvx - \rvy(T)), T)[\rvx] \tran (\rvx - \rvy(T)) \ud t + \int_0^T \vs_{\vtheta^*}(\rvy(t), t)[t] + f(\rvy(t),t)\tran \vs_{\vtheta^*}(\rvy(t), t)[\rvx] \ud t
%     \end{split}
%     \label{eq:pathwise}
% \end{equation}
% since $ \vs_{\vtheta^*}(\rvx, T)[\rvx] \approx \nabla_{\rvx} \log q(\rvx)$.

Note that the pathwise density ratio estimation method in \cref{eq:pathwise} requires 
% joint training of the score model, as we need 
both the time \emph{and} data scores for $p_t(\rvx)$. 
A nice property of our score matching framework is that it makes it easy to incorporate additional, auxiliary information that may be helpful for the downstream task into the training objective in \cref{time_obj} .
% in \cref{time_obj} is that it makes it easy to incorporate additional, auxiliary information that may be helpful in the density ratio estimation task. 
% \kristy{explain why should estimating the data scores help}
Specifically, we can define a vector-valued score model $\vs_\vtheta(\rvx, t)$ and train it with a hybrid objective that seeks to \emph{jointly learn} $\nabla_{[\rvx; t]} \log p(\rvx, t)$:
% the data scores $\nabla_\rvx \log p_t(\rvx)$ as well as the time scores:
\allowdisplaybreaks
\begin{equation}
\label{eqn:joint_obj}
\begin{split}
    \mathcal{L_{\text{joint}}(\theta)} =& \E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\left[ \frac{1}{2}\lambda(t)\norm{\nabla_{[\rvx; t]}\log p(\rvx, t) - \vs_\vtheta(\rvx, t)}_2^2 \right]\\
    =&\E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\left[ \frac{1}{2} \lambda(t) \norm{\vs_\vtheta(\rvx, t)}_2^2 + \lambda(t) \operatorname{tr}(\mJ_{\vs_\vtheta}(\rvx, t)) + \lambda'(t) \vs_\vtheta(\rvx, t)[t] \right] \\
    &+ \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta(\rvx, 0)[t]] - \E_{p_1(\rvx)}[\lambda(1) \vs_\vtheta(\rvx, 1)[t]] + \text{const.}\\
    =&\E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\E_{\rvv \sim \mcal{N}(\bm{0}, \mI)}\left[ \frac{1}{2}\lambda(t) \norm{\vs_\vtheta(\rvx, t)}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta(\rvx, t) \rvv + \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta(\rvx, t)[t] + \lambda'(t) \vs_\vtheta(\rvx, t)[t]\right] \\
    &+ \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta(\rvx, 0)[t]] - \E_{p_1(\rvx)}[\lambda(1) \vs_\vtheta(\rvx, 1)[t]] + \text{const}.
\end{split}
\end{equation}
% \chenlin{i think we might need to clean the eq up }
\chenlin{
Specifically, we can define a vector-valued score model $\vs_\vtheta(\rvx, t)$ and train it with a hybrid objective that seeks to \emph{jointly learn} $\nabla_{[\rvx; t]} \log p(\rvx, t)$:
\begin{equation}
\label{eqn:joint_obj}
    \mathcal{L_{\text{joint}}(\theta)} = \E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\left[ \frac{1}{2}\lambda(t)\norm{\nabla_{[\rvx; t]}\log p(\rvx, t) - \vs_\vtheta(\rvx, t)}_2^2 \right].
\end{equation}
In fact, optimizing \cref{eqn:joint_obj} is equivalent to optimizing the following tractable objective.
\begin{theorem}
The optimal $\theta^*$ that minimize 
\begin{align}
\label{eq:objective_simplified}
    \theta^{*} = \argmin_{\theta} 
    &\E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\E_{\rvv \sim \mcal{N}(\bm{0}, \mI)}\bigg[ \frac{1}{2}\lambda(t) \norm{\vs_\vtheta(\rvx, t)}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta(\rvx, t) \rvv \\
    &+ \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta(\rvx, t)[t]
    + \lambda'(t) \vs_\vtheta(\rvx, t)[t]\bigg]
    + \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta(\rvx, 0)[t]] - \E_{p_1(\rvx)}[\lambda(1) \vs_\vtheta(\rvx, 1)[t].
\end{align}
\end{theorem}
In practice, the expectation in \cref{eq:objective_simplified} can be approximated by finite samples using Monte Carlo estimator.
% write a sample based eq
}
% \begin{align*}
% \label{eqn:joint_obj}
%     &\E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\left[ \frac{1}{2}\lambda(t)\norm{\nabla_{[\rvx; t]}\log p(\rvx, t) - \vs_\vtheta(\rvx, t)}_2^2 \right]\\
%     =&\E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\left[ \frac{1}{2} \lambda(t) \norm{\vs_\vtheta(\rvx, t)}_2^2 + \lambda(t) \operatorname{tr}(\mJ_{\vs_\vtheta}(\rvx, t)) + \lambda'(t) \vs_\vtheta(\rvx, t)[t] \right] \\
%     &+ \frac{1}{T} \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta(\rvx, 0)[t]] - \frac{1}{T}\E_{p_1(\rvx)}[\lambda(T) \vs_\vtheta(\rvx, T)[t]] + \text{const.}\\
%     =&\E_{t \sim \mcal{U}(0, 1)}\E_{\rvx \sim p_{t}(\rvx)}\E_{\rvv \sim \mcal{N}(\bm{0}, \mI)}\left[ \frac{1}{2}\lambda(t) \norm{\vs_\vtheta(\rvx, t)}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta(\rvx, t) \rvv + \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta(\rvx, t)[t] + \lambda'(t) \vs_\vtheta(\rvx, t)[t]\right] \\
%     &+ \frac{1}{T} \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta(\rvx, 0)[t]] - \frac{1}{T}\E_{p_1(\rvx)}[\lambda(T) \vs_\vtheta(\rvx, T)[t]] + \text{const}.
% \end{align*}
% \chenlin{so this is the summation (combination) of score matching loss on x and on t?}
% \chenlin{how do you deal with the cases when score is not well defined if you do not add noise?
%  why not use the dsm version? }

% The optimal score-based model satisfies $\vs_{\vtheta^*}(\rvx, t) \approx [\nabla_\rvx \log p_{t}(\rvx); \partial_t \log p_{t}(\rvx)]$. This is because $\vs_{\vtheta^*}(\rvx, t) \approx \nabla_{[\rvx;t]} \log p(\rvx, t)$ and
% \begin{align*}
%     \nabla_\rvx \log p(\rvx, t) &= \nabla_\rvx \log p_{t}(\rvx) + \nabla_\rvx \log p(t) = \nabla_\rvx \log p_{t}(\rvx)\\
%     \partial_t \log p(\rvx, t) &= \partial_t \log p_{t}(\rvx) + \partial_t \log p(t) = \partial_t \log p_{t}(\rvx),
% \end{align*}
% since $p(t)$ does not depend on $\rvx$ and is a uniform distribution. 

% After training, we let $\vs_\vtheta(\rvx, t)[t]$ denote the last dimension (time dimension) of $\vs_\vtheta(\rvx, t)$, and let $\vs_\vtheta(\rvx, t)[\rvx]$ denote the remaining dimensions. We can estimate the log density ratio through \kristy{this might be redundant}
% \begin{align*}
%     r(\rvx) \approx \int_{0}^T \vs_{\vtheta^*}(\rvx, t)[t] \ud t.
% \end{align*}

To estimate the data scores, which  correspond to the first two terms of \cref{eqn:joint_obj}, we can leverage either DSM or SSM.
% Given \cref{eqn:joint_obj}, we can leverage either the DSM or SSM objectives
% denoising score matching (DSM) \citep{song2019generative} or sliced score matching (SSM) \citep{song2020sliced} objectives 
% to learn the data scores, which correspond to the first two terms of \cref{eqn:joint_obj}. 
For the setting when the underlying SDE is known and $p(\bx) = \mathcal{N}(\bm{0}, \bm{I})$,
% For some choices of $p(\bx)$, 
% for example the standard normal Gaussian as in the MNIST energy-based modeling experiments (for specific choices of the forward SDE), 
we can directly use DSM since we can analytically compute the form of $p_{t}(\bx)$. 
This is desirable because the DSM objective typically exhibits lower variance than that of SSM. However, the SSM objective is beneficial in situations where we can only access the intermediate distributions through samples.
% the form of $p(\bx)$ is unknown, and we can only access it through samples.

In fact, this joint training objective is most useful when one of the densities (e.g. $p(\rvx)$) is known and can be computed in closed form, as in energy based modeling. 
In this setting, the expression $\log p(\rvy) - \log p(\rvx)$ can be computed analytically, bypassing the need to rely on the learned time score network for estimating the second integral in \cref{eq:pathwise}. 
Then, only the first integral needs to be estimated using the learned time and data scores.
% via the time score network and the data score network. 
Since the data scores can be learned fairly well with recent advances in score-based generative models, the estimation of the first integral tends to be more accurate than using the time score network alone. 
% \kristy{clean this up}

The benefits of the pathwise approach is shown in Figure~\ref{fig:2d_exp_shift1}(d), where all models trained on $p(\rvx) = \mcal{N}(\bm{0}, \mI)$ and $q(\rvx) = \mcal{N}(\bm{4}, \mI)$ are evaluated on 10K samples drawn from $\mcal{N}(\bm{0}, \mI)$ and $\mcal{N}(\bm{5}, \mI)$ each.
Although the performance of all models slightly degrades (the baseline NCE is not shown, as it performed extremely poorly), the additional integration path helps the jointly trained score model to more accurately recover the density ratios relative to other methods.
% The performance of all models slightly degrades (the baseline NCE is not shown, as it performed extremely poorly). However, with the line path introduced in this section, the joint score model is able to accurately recover the density ratios. This can be seen in Figure~\ref{fig:2d_exp_shift1}.

% Intuitively, the joint training procedure can be thought of as the score-matching variant of a generative classifier \citep{grathwohl2019your}. That is, we can think of the time scores as roughly corresponding to the score variant of the classifier's output probabilities $p(y|\rvx)$, while the data scores would correspond to the score variant of the class-conditional density $p(\rvx|y)$. We hypothesize that this score matching approach would be a nice way to train a hybrid classifier without the normalizing constant (or training an EBM via SGLD), which we leave to future work. \kristy{maybe we can just take this out}

% \kristy{I think joint training is the continuous relaxation of \citep{grathwohl2019your}. So maybe if we train a classifier in this way, we'll get better calibrated classifiers. Also, this would be a nice way to train a hybrid classifier without the normalizing constant (or training an EBM via SGLD as in \citep{grathwohl2019your})}


\begin{figure*}[!t]
    \centering
        \subfigure[TRE(4) MSE: 8.1]{\includegraphics[width=.25\textwidth]{figures/2d_gmm_shift1/TRE(4).png}}
        \subfigure[TRE(9) MSE: 2.0]{\includegraphics[width=.24\textwidth]{figures/2d_gmm_shift1/TRE(9).png}}
        \subfigure[Time MSE (Ours): 1.1]{\includegraphics[width=.24\textwidth]{figures/2d_gmm_shift1/Time Scores.png}}
        \subfigure[Joint MSE (Ours): 0.6]{\includegraphics[width=.25\textwidth]{figures/2d_gmm_shift1/Joint (Exact).png}}
    \caption{Additional results on the synthetic 2-D Gaussian dataset on a more challenging evaluation task, where half the samples are shifted by 1. While all models' performance slightly degrade, our joint score matching objective still accurately recovers the density ratio estimates.}
    \label{fig:2d_exp_shift1}
\end{figure*}





==> sections/old_method.tex <==
\section{Time Score Matching via Infinitesimal Classification}
\label{method}
% \ys{I suggest the following structure
% \begin{itemize}
%     \item Introduce the concept of time scores by studying the limit of TRE as $T\to\infty$.
%     \item Talk about different ways to bridge two densities. Diffusion processes, general stochastic processes, etc.
%     \item Introduce new methods to estimate the time scores.
% \end{itemize}
% }
\subsection{Discrete Bridges to Continuous Paths}
\label{time_training}
To develop a more scalable alternative to \cref{eq:tre}, 
we propose to \se{why relax?} relax the number of bridges $T \rightarrow \infty$ and consider a continuous \textit{path} of bridge distributions connecting $p_0(\rvx)$ and $p_1(\rvx)$ in distribution space. 
Note that there are two objects \se{challenges?} that we must consider in this limiting case: (1) the behavior of each intermediate classifier in TRE; and (2) the telescoping sum.

\se{it might make the story more interesting if you say that counterintuitively/surprisingly, we actually make $T$ even larger. and that turns out to have computational benefits } 
% \paragraph{Infinitesimal Classifier.} We first study the $t$-th classifier in TRE as the gap ($\Delta t$) between $p_t(\rvx)$ and $p_{t+1}(\rvx)$ becomes infinitesimal.
% Recall that it is trained by optimizing the following cross-entropy loss:
% \begin{multline*}
%     \vtheta^* = \argmax_\vtheta \mathbb{E}_{p_{(t-1)/T}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t/T))] \\ + \mathbb{E}_{p_{t/T}(\rvx)}[\log \vh_\vtheta(\rvx, t/T)],
% \end{multline*}
% where $\vh_\vtheta(\rvx, t/T) \in [0,1]$ is a binary classifier. By calculus of variations, we can derive that for the optimal model parameter $\vtheta^*$,
% \begin{align*}
%     \vh_{\vtheta^*}(\rvx, t/T) = \sigma(\log p_{t/T}(\rvx) - \log p_{(t-1)/T}(\rvx)),
% \end{align*}
% where $\sigma(\rvx) = \frac{1}{1+e^{-\rvx}}$ is the sigmoid function. 
% Thus when $T\to\infty$, we clearly have that:
% \begin{align*}
%     \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} O\left(\dt \log p_t(\rvx)\right).
% \end{align*}
% This expression says that in the limit of $T\to \infty$, the optimal classifier between two infinitesimally close bridges (``infinitesimal classifier'') becomes an expression of how much each intermediate density is changing over time ($\dt \log p_t(\rvx)$). 
% In direct analogy to traditional data (Stein) scores $\nabla_\rvx \log p(\rvx)$, we name this quantity $\dt \log p_t(\rvx)$ the \emph{time score} function of $p_t(\rvx)$.

\paragraph{Infinitesimal Classifier.} We first study the $t$-th classifier in TRE as the gap ($\Delta t$) between $p_t(\rvx)$ and $p_{t+1}(\rvx)$ becomes infinitesimal, which we call an ``infinitesimal classifier.'' Recall that it is trained by optimizing the following cross-entropy loss:
\begin{multline*}
    \vtheta^* = \argmax_\vtheta \mathbb{E}_{p_{(t-1)/T}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t/T))] \\ + \mathbb{E}_{p_{t/T}(\rvx)}[\log \vh_\vtheta(\rvx, t/T)],
\end{multline*}
\se{this eq probably belongs to the TRE background part. here you can work out the limiting behavior}
\se{lots of undefined stuff here. deltat, the cross-entropy loss, the h notation doesn't even match the one from 2.1 where the classifier was c}
where $\vh_\vtheta(\rvx, t/T) \in [0,1]$ is a binary conditional classifier. Then via calculus of variations:
\begin{proposition}
\label{prop:score_clf} When $T \rightarrow \infty$, the form of the optimal classifier between two adjacent bridge distributions $p_{t/T}(\rvx)$ and $p_{(t+1)/T}(\rvx)$ becomes: \kristy{TODO}
\begin{equation}
    \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} O\left(\dt \log p_t(\rvx)\right).
\end{equation}
\end{proposition}
% Recall that it is trained by optimizing the following cross-entropy loss:
% \begin{multline*}
%     \vtheta^* = \argmax_\vtheta \mathbb{E}_{p_{(t-1)/T}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t/T))] \\ + \mathbb{E}_{p_{t/T}(\rvx)}[\log \vh_\vtheta(\rvx, t/T)],
% \end{multline*}
% where $\vh_\vtheta(\rvx, t/T) \in [0,1]$ is a binary classifier. By calculus of variations, we can derive that for the optimal model parameter $\vtheta^*$,
% \begin{align*}
%     \vh_{\vtheta^*}(\rvx, t/T) = \sigma(\log p_{t/T}(\rvx) - \log p_{(t-1)/T}(\rvx)),
% \end{align*}
% where $\sigma(\rvx) = \frac{1}{1+e^{-\rvx}}$ is the sigmoid function. 
% Thus when $T\to\infty$, we clearly have that:
% \begin{align*}
%     \vh_{\vtheta^*}(\rvx, t) = \frac{1}{2} + \frac{1}{4} O\left(\dt \log p_t(\rvx)\right).
% \end{align*}
\se{big O notation doesn't make sense}

\se{give some intuition here. $\frac{\partial}{\partial t} \log p_t(\rvx) \approx \log p_{t+\delta_t}(\rvx)  - \log p_{t}(\rvx) = \log \frac{p_{t+\delta_t}(\rvx)} {p_{t}(\rvx)} $}

This expression says that the form of the optimal infinitesimal classifier becomes an expression of how much each intermediate density is changing over time ($\dt \log p_t(\rvx)$). 
In direct analogy to traditional data (Stein) scores $\nabla_\rvx \log p(\rvx)$, we name this quantity $\dt \log p_t(\rvx)$ the \emph{time score} function of $p_t(\rvx)$.


\paragraph{Integration of Time Scores.} Next, we see that as the number of bridge distributions increase, the telescoping sum becomes an integral \citep{gelman1998simulating,owen2013monte,yao2020adaptive}:
\begin{equation*}
\resizebox{\linewidth}{!}{$
    \begin{split}
    \log \frac{p_0(\rvx)}{p_1(\rvx)} &= \sum_{t=1}^{T} \log \left( \frac{p_{(t-1)/T}(\rvx)}{p_{t/T}(\rvx)} \right) \\
    & \approx \lim_{T \rightarrow \infty} \frac{1}{T} \sum_{t=1}^T \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) \vert_{\lambda=\frac{t}{T}} = \int_{1}^0 \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) d\lambda 
    \end{split}
$}.
\end{equation*}
% This idea is rooted in simulated annealing \citep{jarzynski1997nonequilibrium,neal2001annealed} and path sampling \citep{gelman1998simulating,blanchet2007path,yao2020adaptive}, which are advanced variance reduction techniques for importance sampling in the context of approximating intractable normalizing constants.
This identity has conveniently converted the need to solve $T$ binary classification problems into one that requires the ability to estimate the time scores $\dt \log p_t(\rvx)$ via $\vh_\vtheta(\rvx, t/T)$.
% what you had before
% To develop a more scalable alternative to \cref{eq:tre}, 
% we propose to relax the number of bridges to infinity and consider a continuous \textit{path} of intermediate distributions connecting $p_0(\rvx)$ and $p_1(\rvx)$.
% Then as shown in \citep{gelman1998simulating,owen2013monte,yao2020adaptive}, our telescoping sum is converted into an integral,
% where we integrate over the time scores $\dt \log p_t(\rvx)$ across the entire range of $t \in [0, 1]$:
% \kristy{check last line}
% \ys{We can make this a rigorous statement in a theorem. The proof is clear according to the definition of Riemann integral (assuming continuity).}
% \begin{equation*}
% \resizebox{\linewidth}{!}{$
%     \begin{split}
%     \log \frac{p_0(\rvx)}{p_1(\rvx)} &= \sum_{t=1}^{T} \log \left( \frac{p_{(t-1)/T}(\rvx)}{p_{t/T}(\rvx)} \right) \\
%     & \approx \lim_{T \rightarrow \infty} \frac{1}{T} \sum_{t=1}^T \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) \vert_{\lambda=\frac{t}{T}} = \int_{1}^0 \frac{\partial}{\partial \lambda} \log p_\lambda(\rvx) d\lambda 
%     \end{split}
% $}
% \end{equation*}
% where we let $T$ denote the total number of intermediate bridges.
% % \ys{We can also include a formal statement on how the optimal classifier between nearby bridging distributions become an expression of the time score in the limit of $T\to \infty$. Should be a very interesting result to have.}
% This idea is rooted in simulated annealing \citep{jarzynski1997nonequilibrium,neal2001annealed} and path sampling \citep{gelman1998simulating,blanchet2007path,yao2020adaptive}, which are advanced variance reduction techniques for importance sampling in the context of approximating intractable normalizing constants.
% This identity has conveniently converted the need to solve $K$ binary classification problems into one that requires the ability to estimate the time scores $\dt \log p_t(\rvx)$.
Additionally, the integration over all intermediate time scores in \cref{eqn:dr1} can be computed
using any existing numerical ODE solver. \se{the ODE vs numerical integration is confusing. there is no ODE so far}

The ODE solver determines the timesteps $t$ we should query along the trajectory as we obtain our density ratio estimates, which eliminates its dependence on $T$ as in \cref{eq:tre}.

\subsection{Time Score Estimation}
There are several ways to estimate the time scores from data (without training an infinite number of classifiers), depending on how $q(\rvx)$ and $p(\rvx)$ are bridged together.
% The time score $\dt \log p_t(\rvx)$ is defined analogously to the data score $\nabla_\rvx \log p_t(\rvx)$ (Section~\ref{score_genmo}).
% \begin{definition}[Time Score]
% $\dt \log p_t(\rvx)$ \kristy{TODO}
% \end{definition}
% The way in which we introduce an infinite number of intermediate bridges 
% % via the continuous-time path 
% is reminiscent of how traditional score-based models with SDEs convolve the data distribution with an infinite number of noise scales (Section~\ref{score_genmo}). In fact, the time score $\dt \log p_t(\rvx)$ bears an uncanny resemblance to the data score $\nabla_\rvx \log p_t(\rvx)$, and we make the analogy explicit in this section. 
% , and we make the analogy explicit in this section. 
% \kristy{need a better transition. but introduce the time score here, relate it back to data scores.}
% \kristy{from the intro..}
% \begin{enumerate}
%     \item The time score bears a close similarity to traditional data scores, which measure how a density is changing over its input domain.
%     \item The time score is estimating for each x the instantaneous rate of change of $p_t(\rvx)$ along that path. It measures how each intermediate density is locally changing along a prescribed trajectory over time.
% \end{enumerate}
% \kristy{Because of the analogous way in which the time scores are defined, we can similarly draw inspiration from recent advances in score matching to develop an objective for learning the time scores (this will be tied into the unknown sde section, move stuff). this will also make some background on SM useful in 2.1 with the risk of making the exposition a little long. but the similarity in the derivation (e.g. int by parts) will look v familiar} \kristy{can we tie back to Figure 1 and make the relationship between the 2 scores stronger?}
% \kristy{continuation of what you had before below}
% \ys{Talk about different ways to bridge two densities. Diffusion processes, general stochastic processes, etc.}
\paragraph{Bridge Specification.} 
% In fact, the way in which we introduce an infinite number of intermediate bridges 
% via the continuous-time path 
% is reminiscent of how traditional score-based models with SDEs convolve the data distribution with an infinite number of noise scales. 
% As we draw inspiration from this traditional (Stein) score matching setup, \ys{No need to talk about drawing inspiration from score-based generative models. You can have a related work section to discuss this, but since those are complicated concepts to explain, it's can be confusing to discuss them directly in the main text. It also undermines the novelty of our approach a little bit.}
One such example is a diffusion process, where the data generating process of $q(\rvx)$ is represented as a Markov chain that transforms a simple distribution $p_T(\rvx) \equiv p(\rvx)$
into a target distribution $p_0(\rvx) \equiv q(\rvx)$ \citep{sohl2015deep,ho2020denoising,song2020denoising}. 
% When $L \rightarrow \infty$ \citep{song2020score}, such a probabilistic model represents the data generating process of $p(\rvx)$ with a Markov chain that transforms a simple distribution $p_T(\rvx)$
% into a complex target distribution $p_0(\rvx) \equiv p(\rvx)$ \citep{sohl2015deep,ho2020denoising,song2020denoising}. 
This sequential procedure can be described as the solution to an It$\hat{\textrm{o}}$ stochastic differential equation (SDE):
\[
\dd\rvx = \bff(\rvx, t)\dd t + g(t)\dd \bw
\]
where $\bw$ represents Brownian motion, $\bff(\cdot,t): \mathbb{R}^D \rightarrow \mathbb{R}^D$ is the drift coefficient of $\rvx(t)$, and $g(\cdot): \mathbb{R} \rightarrow \mathbb{R}$ is the diffusion coefficient of $\rvx(t)$, where $\rvx(t) \sim p_t(\rvx)$. 
Intuitively, this equation governs how the intermediate density $p_t(\rvx)$ changes as a function of time and noise \citep{oksendal2003stochastic}, and induces a set of stochastic paths in distribution space $\{\rvx(t)\}_{t \in [0, 1]}$ across timesteps $t$ that connect the initial and target densities together. 
% \kristy{talk about diffusion}
% \kristy{does this part about diffusion models/SDEs seem like it came out of nowhere?}
% We use $\rvx(t)$ to denote a sample from the intermediate distribution $p_t(\rvx)$. 

Although we often cannot access the data distribution's underlying SDE,
there are many ways to specify the intermediate distributions $p_{t}(\rvx)$ given $p(\rvx)$ and $q(\rvx)$.
For example, we can define 
% a sample from $p_{t}(\rvx)$ as 
$\rvx(t) := \sqrt{1-\alpha(t)^2} \rvx + \alpha(t) \rvy$, where $\rvx \sim q$, $\rvy \sim p$, and $\alpha: [0,1] \to \R^+$ is a positive function that satisfies $\alpha(0) = 0$ and $\alpha(1) = 1$. 
A benefit of DRE-$\infty$ is that it is fully general, in that we do not require the data generating process to follow a prescribed SDE or diffusion process;
% a prescribed form of the SDE or even require the data generating process to follow a particular diffusion process; 
our method only requires that we be able to \emph{sample} from all distributions along the spectrum of $q(\rvx)$ and $p(\rvx)$. 

\paragraph{Known SDE/Diffusion process.} For learning settings where our data follows a known SDE, 
% \kristy{is this accurate?}\ys{seems right to me}, 
we can leverage the Fokker-Planck equation \citep{jordan1998variational,oksendal2003stochastic} to transform the data scores $\nabla_\rvx \log p_t(\rvx)$ into time scores \emph{without training an additional model}.
The Fokker-Planck equation describes the time-evolution of the probability density $p_t(\rvx)$ associated with the SDE:
% , and can be used to obtain an estimate of the time scores via a transformation of the data scores $\nabla_\rvx \log p_t(\rvx)$:
\begin{equation}
\label{fokker-planck}
\resizebox{\linewidth}{!}{$
\begin{split}
    \frac{\partial}{\partial t}\log p_t(\rvx) &= -\nabla \cdot \bff - \bff \tran \nabla_\rvx \log p_t(\rvx) \\
    &+ g^2(t) \left[ ||\nabla_\rvx \log p_t(\rvx) ||^2_2 + \textrm{tr}(\nabla_\rvx^2 \log p_t(\rvx)) \right]
\end{split}
$}
\end{equation}
% \chenlin{should it be
% \begin{equation}
%     \frac{\partial}{\partial t}\log p_t(\rvx) = -\nabla \cdot \bff - \bff \tran \nabla_\rvx \log p_t(\rvx) + \frac{g^2(t)}{2} \left[ ||\nabla_\rvx \log p_t(\rvx) ||^2_2 + \textrm{sum}(\nabla_\rvx^2 \log p_t(\rvx)) \right]
% \end{equation}
% divided by $2$ can be removed depending on parameterization.
% }
% \chenlin{can the score on t be derived from data score? yes, but it involves the trace term, which is estimated by hutchison's trace estimator since otherwise it would be too expensive}
where $\bff$ and $g$ are well-defined for tractable SDEs. 
% such as the Variance Preserving SDE (VPSDE) in diffusion probabilistic models.
% With recent advances in score-based generative models, 
% We can train a data score network $s_\vtheta(\rvx, t)$ to approximate $\nabla_\rvx \log p_t(\rvx)$ via \cref{og_ssm} or \cref{og_dsm}. 
We can train a data score network $s_\vtheta^{\textrm{data}}(\rvx, t)$ to approximate $\nabla_\rvx \log p_t(\rvx)$ via sliced score matching (SSM) \citep{song2020sliced} or denoising score matching (DSM) \citep{vincent2011connection,song2019generative}. 
% We can train a data score network $s_\vtheta(\rvx, t)$ to approximate $\nabla_\rvx \log p_t(\rvx)$ with denoising score matching (DSM) \citep{vincent2011connection} or sliced score matching (SSM) \citep{song2020sliced} as in \cref{og_ssm} and \cref{og_dsm} respectively. 
The $\nabla \cdot \bff$ term can be estimated efficiently via the Skilling-Hutchinson trace estimator \citep{skilling1989eigenvalues,hutchinson1989stochastic}.
\se{this part will not be understandable to the reader}
% For computational efficiency, we can leverage the Skilling-Hutchinson trace estimator \citep{skilling1989eigenvalues,hutchinson1989stochastic} to compute $\nabla \cdot \bff$.
% \kristy{todo} The data score $\nabla_\rvx \log p_t(\rvx)$ can be obtained by leveraging recent advances from score-based generative models, either via 
% We note that the quantity $\nabla_\rvx \log p_t(\rvx)$ can be obtained by training a data score network either via 
% denoising score matching (DSM) \citep{vincent2011connection} or sliced score matching (SSM) \citep{song2020sliced}. 

\paragraph{Unknown/Intractable SDE.} 
% In many practical scenarios where we do not know the data distribution's underlying SDE,
% \chenlin{tractable?}
% Although we often cannot access the data distribution's underlying SDE,
% there are many ways to specify the intermediate distributions $p_{t}(\rvx)$ given $p(\rvx)$ and $q(\rvx)$.
% However, many practical scenarios do not have grant us access to the underlying SDE. 
In many practical scenarios where we do not know the data distribution's underlying SDE, we must turn to \textit{learning} the time scores. 
% Our framework is fully general, in the sense that we do not require a prescribed form of the SDE or even require the data generating process to follow a particular diffusion process; our method only requires that we be able to sample from all the distributions along the spectrum of $p_1(\rvx)$ and $p_0(\rvx)$. 
% , or we only have access to \textit{samples} of the intermediate distributions $\log p_t(\rvx)$, or we do not have access to the $\nabla_\rvx \log p_t(\rvx)$. \kristy{clean this up}. \kristy{transition or take out} 
% Note that there are many ways to specify $p_{t}(\rvx)$ given $p(\rvx)$ and $q(\rvx)$ even without specifying an SDE. 
% For example, we can define a sample from $p_{t}(\rvx)$ as $\rvx(t) := \sqrt{1-\alpha(t)^2} \rvx + \alpha(t) \rvy$, where $\rvx \sim q$, $\rvy \sim p$, and $\alpha: [0,1] \to \R^+$ is a positive function that satisfies $\alpha(0) = 0$ and $\alpha(1) = 1$. 
To do so, we consider the limit of the binary cross-entropy loss function for the optimal infinitesimal classifier (\cref{prop:score_clf}) when $T\to \infty$. 
% Recall from Section~\ref{time_training} that the optimal ``infinitesimal classifier" is a function of the time score.
% We consider the limit of the binary cross-entropy loss function when $T\to \infty$. 
% \kristy{The training of this "infinitesimal classifier" naturally lends itself to a time score matching objective.}
\begin{proposition}
\label{prop:opt_clf}
Let $\Delta t = 1/T$ and parameterize the binary classifier as $\vh_\vtheta(\rvx, t) = \frac{1}{2} + \frac{1}{4} \vs_\vtheta^{\textrm{time}}(\rvx, t)\Delta t$, where $\vs_\vtheta^{\textrm{time}}(\rvx, t) \approx \dt \log p_t(\rvx)$ denotes a time score model. Then from the binary cross-entropy objective:
\begin{equation}
% \label{eq:loss}
\resizebox{\linewidth}{!}{$
\begin{split}
    &\mathbb{E}_{p_{t}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t))] + \mathbb{E}_{p_{t+\Delta t}(\rvx)}[\log \vh_\vtheta(\rvx, t)]\\
    =& -\frac{1}{4} (\Delta t)^2 \mbb{E}_{p_t(\rvx)}\left[\norm{\vs_\vtheta^{\textrm{time}}(\rvx, t) - \dt \log p_t(\rvx)}_2^2\right] + o((\Delta t)^2)
\end{split}
$}
\end{equation}
\end{proposition}
% \begin{align*}
%     &\mathbb{E}_{p_{t}(\rvx)}[\log (1 - \vh_\vtheta(\rvx, t))] + \mathbb{E}_{p_{t+\Delta t}(\rvx)}[\log \vh_\vtheta(\rvx, t)]\\
%     =& -2\log 2 + \frac{1}{2}\Delta t \int (p_{t+\Delta t}(\rvx) - p_t(\rvx))\vs_\vtheta(\rvx, t) \ud \rvx \\
%     & -\frac{1}{4} (\Delta t)^2 \mathbb{E}_{p_t(\rvx)}[\vs_\vtheta(\rvx, t)^2]+ o((\Delta t)^2)\\
%     =& -2\log 2 + \frac{1}{2}(\Delta t)^2 \mbb{E}_{p_t(\rvx)}\left[\dt \log p_t(\rvx) \vs_\vtheta(\rvx, t)\right] \\
%     & -\frac{1}{4} (\Delta t)^2 \mathbb{E}_{p_t(\rvx)}[\vs_\vtheta(\rvx, t)^2]+ o((\Delta t)^2)\\
%     =& -\frac{1}{4} (\Delta t)^2 \mbb{E}_{p_t(\rvx)}\left[\norm{\vs_\vtheta(\rvx, t) - \dt \log p_t(\rvx)}_2^2\right] + o((\Delta t)^2) + \text{const}.
% \end{align*}
We defer the proof to Appendix~\ref{pf-opt-clf}.


% what you had before
% In such a setting, we must turn to \textit{learning} the time scores. With an interpolation mechanism in place, we propose to train a time score model $s_\vtheta(\rvx, t)$ with the following time score matching objective:
Therefore, we see that the training of this infinitesimal classifier naturally lends itself to the following time score matching objective. We use this expression to train a time score model $s_\vtheta^{\textrm{time}}(\rvx, t)$:
\begin{equation}
\label{time_obj}
\resizebox{\linewidth}{!}{$
\begin{split}
        \mathcal{J_{\text{time}}(\theta)} &= \E_{p(t)}\E_{p_t(\rvx)}\bigg[\lambda(t) \left( \dt \log p_t(\rvx) - s_\vtheta^{\textrm{time}}(\rvx, t) \right)^2 \bigg]
\end{split}
$}
\end{equation}
% \chenlin{$s_\vtheta(\rvx, t)$ is time score or data score? have you introduced this notation?}
% \chenlin{consider writing is as
% \begin{equation}
% \label{time_obj}
% \resizebox{\linewidth}{!}{$
% \begin{split}
%         \mathcal{J_{\text{time}}(\theta)} &= \E_{t}\E_{\rvx }\bigg[\lambda(t) \left( \dt \log p_t(\rvx) - s_\vtheta(\rvx, t) \right)^2 \bigg],
% \end{split}
% $}
% \end{equation}
% $t\sim \mcal{U}, \rvx \sim p_{t}(\rvx)$
% }
% We note that this expression is directly analogous to the original score matching objective in \cref{og_sm}. 
Thus using integration by parts as in \citep{hyvarinen2005estimation}, we can show that this objective for learning $\dt \log p_t(\rvx)$ can be simplified to the following.

\begin{proposition}[Informal]
\label{prop:time_objective}
Under certain regularity conditions, the optimal solution $\theta^{*}$ of \cref{time_obj} is the same as the optimal solution of
\begin{equation}
\resizebox{\linewidth}{!}{$
\begin{split}
        &\mathcal{L_{\text{time}}(\theta)} = 2 \E_{q(\rvx)}[\lambda(0) s_\vtheta^{\textrm{time}}(\rvx, 0)] - 2\E_{p(\rvx)}[\lambda(1) s_\vtheta^{\textrm{time}}(\rvx, 1)] \\
    &+\E_{p(t)}\E_{p_t(\rvx)}\bigg[2 \lambda(t) \dt s_\vtheta^{\textrm{time}}(\rvx, t) + 2\lambda'(t) s_\vtheta^{\textrm{time}}(\rvx, t) + \lambda(t) s_\vtheta^{\textrm{time}}(\rvx, t)\bigg]
\end{split}
$}
\end{equation}
\end{proposition}
% \allowdisplaybreaks
% \begin{equation}
% \label{time_obj}
% \resizebox{\linewidth}{!}{
% \begin{split}
%         \mathcal{L_{\text{time}}(\theta)} &= \E_{p(t)}\E_{p_t(\rvx)}\bigg[\lambda(t) \left( \dt \log p_t(\rvx) - s_\vtheta(\rvx, t) \right)^2 \bigg] \\
%     &= 2 \E_q[\lambda(0) s_\vtheta(\rvx, 0)] - 2\E_p[\lambda(1) s_\vtheta(\rvx, 1)]\\
%     &+\E_{p(t)}\E_{p_t(\rvx)}\bigg[2 \lambda(t) \dt s_\vtheta(\rvx, t) + 2\lambda'(t) s_\vtheta(\rvx, t) \\
%     &+ \lambda(t) s_\vtheta^2(\rvx, t)\bigg] + \textnormal{const.}
% \end{split}
% }
% \end{equation}
where the first two terms of \cref{prop:time_objective} denote the boundary conditions for $t=\{0,1\}$, and the expectations can be approximated via Monte Carlo sampling. 
We defer the exact assumptions and proof to Appendix~\ref{pf-time-prop}.

% \chenlin{do we plan to mention how we perform reweighting somewhere?}


\subsection{Joint Training Objective}
% \chenlin{does not seem to be in the right section? it does not invole pathwise dre?} \kristy{the logical connection is: pathwise requires data scores; our framework lets us get data scores easily via the joint objective}
%We know that the optimal score-based model satisfies $\vs_{\vtheta^*}(\rvx, t) \approx [\nabla_\rvx \log p_{t}(\rvx); \partial_t \log p_{t}(\rvx)]$. Therefore, for the expression $\log q(\rvy) - \log p(\rvx)$, we have:
% \begin{align*}
%     \log q(\rvy) - \log p(\rvx) \approx \int_0^T \vs_{\vtheta^*}(\rvy(t), t)[t] + f(\rvy(t),t)
%     \tran \vs_{\vtheta^*}(\rvy(t), t)[\rvx] \ud t
% \end{align*}
% which means for the final density ratio estimate we have:
% \begin{equation}
%     \begin{split}
%   r(\rvx) &\approx \int_0^1 \nabla_\rvx \log q(\rvy + t(\rvx - \rvy))\tran (\rvx - \rvy) \ud t + \int_0^T \vs_{\vtheta^*}(\rvy(t), t)[t] + f(\rvy(t),t)\tran \vs_{\vtheta^*}(\rvy(t), t)[\rvx] \ud t \\
%   &\approx \int_0^1 \vs_{\vtheta^*}(\rvy(T) + t(\rvx - \rvy(T)), T)[\rvx] \tran (\rvx - \rvy(T)) \ud t + \int_0^T \vs_{\vtheta^*}(\rvy(t), t)[t] + f(\rvy(t),t)\tran \vs_{\vtheta^*}(\rvy(t), t)[\rvx] \ud t
%     \end{split}
%     \label{eq:pathwise}
% \end{equation}
% since $ \vs_{\vtheta^*}(\rvx, T)[\rvx] \approx \nabla_{\rvx} \log q(\rvx)$.

% Note that the pathwise method in \cref{eq:pathwise} requires 
% % joint training of the score model, as we need 
% both the time \emph{and} data scores for $p_t(\rvx)$. 
% This is not a problem, as another nice property of our time score matching framework is that it makes it easy to incorporate
We can also incorporate
helpful auxiliary information from the data scores
% that may be helpful for the downstream task 
into the training objective in \cref{time_obj}.
Specifically, we can define a vector-valued score model $\vs_\vtheta^{\textrm{joint}}(\rvx, t)$ and train it with a hybrid objective that seeks to \emph{jointly learn} $\nabla_{[\rvx; t]} \log p(\rvx, t)$:
\begin{equation}
\label{eqn:joint_obj}
\resizebox{\linewidth}{!}{$
        \mathcal{J_{\text{joint}}(\theta)} =
        \E_{p(t)}\E_{p_{t}(\rvx)}\left[ \frac{1}{2}\lambda(t)\norm{\nabla_{[\rvx; t]}\log p(\rvx, t) - \vs_\vtheta^{\textrm{joint}}(\rvx, t)}_2^2 \right].
$}
\end{equation}
% We again note the direct correspondence of estimating the data score component in \cref{eqn:joint_obj} to DSM \citep{vincent2011connection} (\cref{og_dsm}) or SSM \citep{song2020sliced} (\cref{og_ssm}).
We again note that the data score component in \cref{eqn:joint_obj} can be obtained by DSM \citep{vincent2011connection} or SSM \citep{song2020sliced}.
% To estimate the data score component $\nabla_\rvx \log p_t(\rvx)$, we can leverage either DSM \citep{vincent2011connection} or SSM \citep{song2020sliced}.
% Given \cref{eqn:joint_obj}, we can leverage either the DSM or SSM objectives
% denoising score matching (DSM) \citep{song2019generative} or sliced score matching (SSM) \citep{song2020sliced} objectives 
% to learn the data scores, which correspond to the first two terms of \cref{eqn:joint_obj}. 
For the SSM variant, following \citep{hyvarinen2005estimation,song2020sliced} shows that optimizing \cref{eqn:joint_obj} is equivalent to the optimizing following objective.
% \chenlin{can maybe say $L_{joint}=L_{ssm}+L_{tim}$ or just say plug in \cref{eq:loss} and apply ssm on the data score?}
\begin{theorem}[Informal]
\label{thm:objective}
Under certain regularity conditions, the solution to the optimization problem in \cref{eqn:joint_obj} can be written as follows:
% \chenlin{you can use resize box}
\begin{equation}
\label{eq:objective_simplified}
\resizebox{0.9\hsize}{!}{$
\begin{split}
    &\theta^{*} = \argmin_{\theta} \textrm{}
    \E_{p(t)}\E_{p_{t}(\rvx)}\E_{p({\rvv})}\bigg[ \\
    &\frac{1}{2}\lambda(t) \norm{\vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx]}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx] \rvv \\
    &+ \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta^{\textrm{joint}}(\rvx, t)[t] + \lambda'(t) \vs_\vtheta^{\textrm{joint}}(\rvx, t)[t]\bigg] \\
    &+ \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta^{\textrm{joint}}(\rvx, 0)[t]] - \E_{p_1(\rvx)}[\lambda(1) \vs_\vtheta^{\textrm{joint}}(\rvx, 1)[t]].
\end{split}
$}
\end{equation}
\end{theorem}
where $\rvv \sim p(\rvv) = \mathcal{N}(\bm{0}, \bm{I})$, $\vs_\vtheta^{\textrm{joint}}(\rvx, t)[\rvx]$ denotes the data score component of $\vs_\vtheta^{\textrm{joint}}$, and $\vs_\vtheta^{\textrm{joint}}(\rvx, t)[t]$ denotes the time-score component of $\vs_\vtheta^{\textrm{joint}}$.
% \kristy{distribution of $\rvv$}
We defer the proof and detailed assumptions to Appendix~\ref{app-joint-proof}. In practice, the expectation in \cref{eq:objective_simplified} can be approximated via Monte Carlo sampling.
This objective is beneficial in situations where we can only sample from 
the intermediate densities $p_t(\rvx)$.
However, we can leverage DSM when
the SDE is known and $p(\bx) = \mathcal{N}(\bm{0}, \bm{I})$
% For some choices of $p(\bx)$, 
% for example the standard normal Gaussian as in the MNIST energy-based modeling experiments (for specific choices of the forward SDE), 
% we can directly use DSM 
since the analytical form of $p_{t}(\bx)$ is tractable. 
\kristy{TODO: mention pseudocode in Appendix~\ref{app-pseudo}}
\kristy{organize when to use what}

\se{i feel there is too much stuff in this section 3. we need to break it up into more manageable chunks for the reader benefit.}
% \cc{doesn't seem clear/obvious when/why we would use the time objective vs the x and time objective}
% This is desirable because the DSM objective typically exhibits lower variance than that of SSM.
% However, the SSM objective is beneficial in situations where we can only sample from the intermediate densities $p_t(\rvx)$.
% \chenlin{add specific equation}\kristy{meh}
% by finite samples using Monte Carlo sampling. 
% We note that after training, the optimal score-based model satisfies $\vs_{\vtheta^*}(\rvx, t) \approx [\nabla_\rvx \log p_{t}(\rvx); \partial_t \log p_{t}(\rvx)]$. This is because $\vs_{\vtheta^*}(\rvx, t) \approx \nabla_{[\rvx;t]} \log p(\rvx, t)$ and
% \begin{align*}
%     \nabla_\rvx \log p(\rvx, t) &= \nabla_\rvx \log p_{t}(\rvx) + \nabla_\rvx \log p(t) = \nabla_\rvx \log p_{t}(\rvx)\\
%     \partial_t \log p(\rvx, t) &= \partial_t \log p_{t}(\rvx) + \partial_t \log p(t) = \partial_t \log p_{t}(\rvx),
% \end{align*}
% since $p(t)$ is uniform with no dependence on $\rvx$. 
% write a sample based eq
% \begin{align*}
% \label{eqn:joint_obj}
%     &\E_{p(t)}\E_{p_{t}(\rvx)}\left[ \frac{1}{2}\lambda(t)\norm{\nabla_{[\rvx; t]}\log p(\rvx, t) - \vs_\vtheta(\rvx, t)}_2^2 \right]\\
%     =&\E_{p(t)}\E_{p_{t}(\rvx)}\left[ \frac{1}{2} \lambda(t) \norm{\vs_\vtheta(\rvx, t)}_2^2 + \lambda(t) \operatorname{tr}(\mJ_{\vs_\vtheta}(\rvx, t)) + \lambda'(t) \vs_\vtheta(\rvx, t)[t] \right] \\
%     &+ \frac{1}{T} \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta(\rvx, 0)[t]] - \frac{1}{T}\E_{p_1(\rvx)}[\lambda(T) \vs_\vtheta(\rvx, T)[t]] + \text{const.}\\
%     =&\E_{p(t)}\E_{p_{t}(\rvx)}\E_{p({\rvv})}\left[ \frac{1}{2}\lambda(t) \norm{\vs_\vtheta(\rvx, t)}_2^2 + \lambda(t) \rvv\tran \nabla_{\rvx} \vs_\vtheta(\rvx, t) \rvv + \lambda(t) \frac{\partial}{\partial t}\vs_\vtheta(\rvx, t)[t] + \lambda'(t) \vs_\vtheta(\rvx, t)[t]\right] \\
%     &+ \frac{1}{T} \E_{p_0(\rvx)}[\lambda(0) \vs_\vtheta(\rvx, 0)[t]] - \frac{1}{T}\E_{p_1(\rvx)}[\lambda(T) \vs_\vtheta(\rvx, T)[t]] + \text{const}.
% \end{align*}
% \chenlin{so this is the summation (combination) of score matching loss on x and on t?}
% \chenlin{how do you deal with the cases when score is not well defined if you do not add noise?
%  why not use the dsm version? }

% The optimal score-based model satisfies $\vs_{\vtheta^*}(\rvx, t) \approx [\nabla_\rvx \log p_{t}(\rvx); \partial_t \log p_{t}(\rvx)]$. This is because $\vs_{\vtheta^*}(\rvx, t) \approx \nabla_{[\rvx;t]} \log p(\rvx, t)$ and
% \begin{align*}
%     \nabla_\rvx \log p(\rvx, t) &= \nabla_\rvx \log p_{t}(\rvx) + \nabla_\rvx \log p(t) = \nabla_\rvx \log p_{t}(\rvx)\\
%     \partial_t \log p(\rvx, t) &= \partial_t \log p_{t}(\rvx) + \partial_t \log p(t) = \partial_t \log p_{t}(\rvx),
% \end{align*}
% since $p(t)$ does not depend on $\rvx$ and is a uniform distribution. 

% After training, we let $\vs_\vtheta(\rvx, t)[t]$ denote the last dimension (time dimension) of $\vs_\vtheta(\rvx, t)$, and let $\vs_\vtheta(\rvx, t)[\rvx]$ denote the remaining dimensions. We can estimate the log density ratio through \kristy{this might be redundant}
% \begin{align*}
%     r(\rvx) \approx \int_{0}^T \vs_{\vtheta^*}(\rvx, t)[t] \ud t.
% \end{align*}

% To estimate the data scores, which  correspond to the first two terms of \cref{thm:objective}, we can leverage either DSM \citep{vincent2011connection} or SSM \citep{song2020sliced}.
% % Given \cref{eqn:joint_obj}, we can leverage either the DSM or SSM objectives
% % denoising score matching (DSM) \citep{song2019generative} or sliced score matching (SSM) \citep{song2020sliced} objectives 
% % to learn the data scores, which correspond to the first two terms of \cref{eqn:joint_obj}. 
% For the setting when the underlying SDE is known and $p(\bx) = \mathcal{N}(\bm{0}, \bm{I})$,
% % For some choices of $p(\bx)$, 
% % for example the standard normal Gaussian as in the MNIST energy-based modeling experiments (for specific choices of the forward SDE), 
% we can directly use DSM since we can analytically compute the form of $p_{t}(\bx)$. 
% This is desirable because the DSM objective typically exhibits lower variance than that of SSM. However, the SSM objective is beneficial in situations where we can only sample from the intermediate densities $p_t(\rvx)$.

% In fact, this joint training objective is most useful when one of the densities (e.g. $p(\rvx)$) is known and can be computed in closed form, as in energy based modeling. 
% In this setting, the expression $\log p(\rvy) - \log p(\rvx)$ can be computed analytically, bypassing the need to rely on the learned time score network for estimating the second integral in \cref{eq:pathwise}. 
% Then, only the first integral needs to be estimated using the learned time and data scores.
% % via the time score network and the data score network. 
% Since the data scores can be learned fairly well with recent advances in score-based generative models, the estimation of the first integral tends to be more accurate than using the time score network alone. 
% % \kristy{clean this up}


